Fault Tolerant Neural Control Barrier Functions for Robotic Systems under Sensor Faults and Attacks

Safety is a fundamental requirement of many robotic systems. Control barrier function (CBF)-based approaches have been proposed to guarantee the safety of robotic systems. However, the effectiveness of these approaches highly relies on the choice of CBFs. Inspired by the universal approximation power of neural networks, there is a growing trend toward representing CBFs using neural networks, leading to the notion of neural CBFs (NCBFs). Current NCBFs, however, are trained and deployed in benign environments, making them ineffective for scenarios where robotic systems experience sensor faults and attacks. In this paper, we study safety-critical control synthesis for robotic systems under sensor faults and attacks. Our main contribution is the development and synthesis of a new class of CBFs that we term fault tolerant neural control barrier function (FT-NCBF). We derive the necessary and sufficient conditions for FT-NCBFs to guarantee safety, and develop a data-driven method to learn FT-NCBFs by minimizing a loss function constructed using the derived conditions. Using the learned FT-NCBF, we synthesize a control input and formally prove the safety guarantee provided by our approach. We demonstrate our proposed approach using two case studies: obstacle avoidance problem for an autonomous mobile robot and spacecraft rendezvous problem, with code available via https://github.com/HongchaoZhang-HZ/FTNCBF.

==> backup/FTSNCBF.tex <==
\section{Fault Tolerant NCBF}
% In this section we present the stochastic NCBFs (SNCBFs) and fault-tolerant SNCBFs (FT-SNCBFs). 
In this section, we first give some background including the Extended Kalman Filter (EKF) and Stochastic CBFs (SCBFs). We next present an overview of the proposed method. Then, we demonstrate the theoretical foundation of SNCBFs and FT-SNCBFs. With the theories support, we present the training process and formulation fault-tolerant framework when deploying

% Background
% EKF
% SCBF
% FT-framework

% High level intuition
% (make sure that the details of overview will be coverd in the later subsections or can be found in other references)

% Synthesis of SNCBF (Training)
% theoretical foundation provide the criterion on what are good SNCBFs
% - correctness (how to check)
% - feasibility (derive condition for SNCBF feasibility)
% Training (Loss function design)
% Based on theroetical foundation, we design the loss function to guide SNCBF to converge

% Synthesis of FT-SNCBF 
% Fault-tolerent is an extension of SNCBF

% FT-Framework (Controller synthesis)
% EKF banks FT-framework
% Safety guarantee

\subsection{Background}
\subsubsection{Extended Kalman Filter}
\begin{assumption}
\label{assumption:ekf}
The SDEs (\ref{eq:state-sde}) and (\ref{eq:output-sde}) satisfy the conditions:
\begin{enumerate}
\item There exist constants $\beta_{1}$ and $\beta_{2}$ such that $\mathbf{E}(\sigma_{t}\sigma_{t}^{T}) \geq \beta_{1} I$ and $\mathbf{E}(\nu_{t}\nu_{t}^{T}) \geq \beta_{2} I$ for all $t$. 
\item The pair $[\frac{\partial \overline{f}}{\partial x}(x,u),c]$ is uniformly detectable.
% \item The system has $(p-1)$ redundancy, where $p>1$. 
\item Let $\phi$ be defined by $$\overline{f}(x,u)-\overline{f}(\hat{x},u) = \frac{\partial \overline{f}}{\partial x}(x - \hat{x}) + \phi(x,\hat{x},u).$$ Then there exist real numbers $k_{\phi}$ and $\epsilon_{\phi}$ such that $$||\phi(x,\hat{x},u)|| \leq k_{\phi}||x-\hat{x}||_{2}^{2}$$ for all $x$ and $\hat{x}$ satisfying $||x-\hat{x}||_{2} \leq \epsilon_{\phi}$. 
\end{enumerate}
\end{assumption} 

\begin{theorem}[\cite{reif2000stochastic}]
\label{theorem:EKF}
Suppose that the conditions of Assumption \ref{assumption:ekf} hold. Then there exists $\delta > 0$ such that $\sigma_{t}\sigma_{t}^{T} \leq \delta I$ and $\nu_{t}\nu_{t}^{T} \leq \delta I$. For any $0<\epsilon <1$, there exists $\gamma > 0$ such that $$Pr\left(\sup_{t \geq 0}{||x_{t}-\hat{x}_{t}||_{2} \leq \gamma}\right) \geq 1-\epsilon.$$ 
\end{theorem}

\subsubsection{Stochastic CBFs}
\begin{theorem}[\cite{clark2020control}]
\label{theorem:SCBF}
    For a system (\ref{eq:state-sde})--(\ref{eq:output-sde}) with safety region defined by (\ref{eq:safe-region}), define
    $$\overline{b}^{\gamma} = \sup_{x,x^{0}}{\{b(\hat{x}) : ||x-x^{0}||_{2} \leq \gamma \text{ and } b(x^{0})=0\}}. $$
    Let $\hat{b}(\hat{x}) := b(\hat{x})-\overline{b}^{\gamma}$. Let $\hat{x}_{t}$ denote the EKF estimate of $x_{t}$, and suppose that there exists a constant $\delta > 0$ such that   
    whenever $\hat{b}(\hat{x}_{t}) < \delta$, $u_{t}$ is chosen to satisfy
    \begin{multline}
    \label{eq:SCBF-2}
    \frac{\partial b}{\partial x}(\hat{x}_{t})\overline{f}(\hat{x}_{t},u_{t}) - \gamma||\frac{\partial b}{\partial x}(\hat{x}_{t})K_{t}c||_{2} \\
    + \frac{1}{2}\mathbf{tr}\left(\nu_{t}^{T}K_{t}^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x}_{t})K_{t}\nu_{t}\right) \geq -\hat{b}(\hat{x}_{t}).
    \end{multline}
    Then $Pr(x_{t} \in \mathcal{D} \ \forall t | \ ||x_{t}-\hat{x}_{t}||_{2} \leq \gamma \ \forall t) = 1$. 
\end{theorem}

% The proof of Theorem \ref{theorem:SCBF} is very similar to the proof of Theorem 7 from \cite{clark2021control} and is omitted due to space constraints.
Intuitively,  Eq. (\ref{eq:SCBF-2}) implies that as the state approaches the boundary, the control input is chosen such that the rate of increase of the barrier function decreases to zero. Hence Theorem \ref{theorem:SCBF} implies that if there exists an SCBF for a system, then the safety condition is satisfied with probability $(1-\epsilon)$ when an EKF is used as an estimator and the control input is chosen at each time $t$ to satisfy (\ref{eq:SCBF-2}).

\begin{definition}[SCBF]
\label{Def:SCBF}
    The function $h$ is a \emph{Stochastic Control Barrier Function (SCBF)} of the system, if for all $\hat{x}_t$ satisfying $h(\hat{x}_t)>0$ there exists $u_t$ s.t. $\forall z_t$ with $\|z_t\|\leq \gamma$ \eqref{eq:SCBF-2} is satisfied. 
\end{definition}

% \subsubsection{Fault Tolerant Safe Control}
% We then select parameters $\gamma_{1},\ldots,\gamma_{m} \in \mathbb{R}_{+}$, and $\{\theta_{ij} : i < j\} \subseteq \mathbb{R}_{+}$, $\delta > 0$. %,  a collection of functions $B_{1},\ldots,B_{m}: \mathbb{R}^{n} \rightarrow \mathbb{R}$, and a collection of class-K functions $\alpha_{3}^{i} : i=1,\ldots,m$. 
% The set of feasible control actions is defined at each time $t$ using the following steps:
% \begin{enumerate}
% \item Define $X_{t}(\delta) = \{i : \hat{h}_{i}(\hat{x}_{t,i}) < \delta\}$. Let $Z_{t} = X_{t}(\delta)$. Define a collection of sets $\Omega_{i}$, $i \in Z_{t}$, by  
% \begin{multline}%{rCl}
% %\nonumber
% \Omega_{i} 
% \triangleq \left\{u: \frac{\partial h_{i}}{\partial x}(\hat{x}_{t,i})\overline{f}(\hat{x}_{t,i},u_{t}) - \gamma_{i}||\frac{\partial h}{\partial x}(\hat{x}_{t,i})K_{t,i}c||_{2}\right.  \\
% \label{eq:FTCBF-constraints}
%  \left.+ \frac{1}{2}\mathbf{tr}(\overline{\nu}_{t,i}^{T}K_{t,i}^{T}\frac{\partial^{2}h_{i}}{\partial x^{2}}(\hat{x}_{t,i})K_{t,i}\overline{\nu}_{t,i}) \geq -\hat{h}_{i}(\hat{x}_{t,i})\right\}. %\IEEEeqnarraynumspace
% \end{multline}
%  Select  $u_{t}$ satisfying $u_{t} \in \bigcap_{i \in X_{t}(\delta)}{\Omega_{i}}$. If no such $u_{t}$ exists, then go to Step 2.
% \item For each $i,j$ with $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} > \theta_{ij}$, set $Z_{t} = Z_{t} \setminus \{i\}$ (resp. $Z_{t} = Z_{t} \setminus \{j\}$) if $||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} > \theta_{ij}/2$ (resp. $||\hat{x}_{t,j}-\hat{x}_{t,i,j}||_{2} > \theta_{ij}/2$).
%   If  $\bigcap_{i \in Z_{t}}{\Omega_{i}} \neq \emptyset$,  then select $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$. Else go to Step 3.
% \item Remove the indices $i$ from $Z_{t}$ corresponding to the estimators with the largest residue values $\overline{y}_{t,i}-\overline{c}_{i}\hat{x}_{t,i}$ until there exists $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$.
% \end{enumerate}
% This policy aims to select a control input that guarantees safety regardless of the fault pattern that is experienced (Step 1). If no such input exists, then the set of constraints is pruned by looking for constraints $\Omega_{i}$ such that  $\hat{x}_{t,i}$ deviates from  $\hat{x}_{t,i,j}$ by more than a threshold value, since such deviations are likely to be due to faults. Meanwhile, if the fault pattern is $r_{i}$, then the estimates $\hat{x}_{t,i}$ and $\hat{x}_{t,i,j}$ will likely be close to one another for all $t$ and $j \neq i$, since both estimators do not rely on the faulted sensor. We note that these constraints are compatible with feedback policies as well as more general history-based control policies. 

% % \begin{theorem}
% % \label{theorem:FT-CBF}
% % Define 
% % \begin{multline*}
% % \overline{h}^{\gamma_{i}} 
% % = \sup{\left\{h(x) : ||x-x^{0}||_{2} \leq \gamma_{i}\right.} \\
% % \left. \mbox{ for some } x^{0} \in h^{-1}(\{0\})\right\}
% % \end{multline*}
% %  and $\hat{h}_{i}(x) = h(x)-\overline{h}^{\gamma_{i}}$. 
% % Suppose  $\gamma_{1},\ldots,\gamma_{m}$, and $\theta_{ij}$ for $i < j$ are chosen such that the following conditions are satisfied:
% % \begin{enumerate}
% % %\item   There exist class-K functions $\alpha_{1}^{i}$, $\alpha_{2}^{i}$: $i=1,\ldots,m$ such that 
% % %\begin{equation}
% % %\label{eq:FT-CBF1}
% % %\frac{1}{\alpha_{1}^{i}(\hat{h}_{i}(x))} \leq B_{i}(x) \leq \frac{1}{\alpha_{2}^{i}(\hat{h}_{i}(x))}.
% % %\end{equation}
% % %for all $x \in \mbox{int}(\mathcal{C})$
% % \item Define  $\Lambda_{i}(\hat{x}_{t,i}) = \frac{\partial h_{i}}{\partial x}(\hat{x}_{t,i})g(\hat{x}_{t,i})$. There exists $\delta > 0$ such that for any $X_{t}^{\prime} \subseteq X_{t}(\delta)$ satisfying $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} \leq \theta_{ij}$ for all $i,j \in X_{t}^{\prime}$,  there exists $u$ such that
% % \begin{equation}
% % \label{eq:FT-CBF2}
% % \Lambda_{i}(\hat{x}_{t,i})u > 0
% % \end{equation}
% % for all $i \in X_{t}^{\prime}$.
% % \item For each $i$, when $r=r_{i}$, 
% % \begin{multline}
% % \label{eq:FT-CBF3}
% % Pr(||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \theta_{ij}/2 \ \forall j, ||\hat{x}_{t,i}-x_{t}||_{2} \leq \gamma_{i} \ \forall t)\\
% %  \geq 1-\epsilon.
% % \end{multline}
% % \end{enumerate}
% % Then $Pr(x_{t} \in \mathcal{C} \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$.
% % \end{theorem}


\subsection{Overview}
% High level intuition
% (make sure that the details of overview will be coverd in the later subsections or can be found in other references)
Our goal is to synthesize a NCBF to play the role of SCBFs. To let one NCBF to replace the SCBFs corresponding to all possible fault patterns, we want to introduce the reasoning component as an input. The reasoning input belongs to a discrete space, indicating the fault patterns $I\in \mathcal{I}$, where $\mathcal{I}$ is the set of all possible fault patterns. To verify the FT-NCBF we verify $b_{\theta}(x\mid I)$, $\forall I\in \mathcal{I}$ where $I$ is the discrete input of fault patterns. 
% \textcolor{blue}{Chain of thought: We split the task into pieces, namely CBFs, stochastic components and conflict resolution. We want the NCBFs to be correct and feasible, so we use incorporate stochastic components while training. However, we eventually need only one NCBF and construct NCBF constraints based on corresponding masks of sensors. Therefore, the overall structure can be NCBF embedded constraints reconfigured by a conflict resolution component. }
In what follows, we will demonstrate our design of the pipeline. 


\subsection{Synthesis of SNCBF}
% Synthesis of SNCBF (Training)
% theoretical foundation provide the criterion on what are good SNCBFs
% - correctness (how to check)
% - feasibility (derive condition for SNCBF feasibility)
% Training (Loss function design)
% Based on theroetical foundation, we design the loss function to guide SNCBF to converge

% We generate with $b_{\theta}(x)$ with sensor noise and under different fault patterns. 

% Theorem to define a valid SCBF for polyCBF and NCBF
In what follows, we describe how to synthesize stochastic neural CBFs (SNCBFs). We first introduce the SCBFs, among which SNCBFs constitute a special class represented by neural networks. 
% The safety of a stochastic system can be ensured safe by Theorem \ref{theorem:SCBF} given a function $b(x)$. In what follows, we shows criterion for SCBF candidates. 
% Let the estimation error to be represented as $z_t = (x_t-\hat{x}_t)$. 
The following proposition gives the  necessary and sufficient conditions for a function $b$ to be a SCBF.  
\begin{proposition}
\label{prop:verify_scbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $b(\hat{x})$ is a SCBF if and only if there is no $\hat{x}\in \mathcal{D}^{\gamma}:=\{\hat{x}\mid \hat{b}_{\theta}^{\gamma}(\hat{x})\geq 0\}$, satisfying
$\frac{\partial b}{\partial x}g(\hat{x}) = 0$ and $\xi(\hat{x}) < 0$, where 
\begin{multline}
\label{eq:prop2cond}
    \xi(\hat{x}) =  \frac{\partial b}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x})K\nu\right) + \\
    ||\frac{\partial b}{\partial x}(\hat{x}_{t,i})K_{t,i}c||_{2} +  \hat{b}(\hat{x}).
\end{multline}
\end{proposition}
The proposition is derived based on \cite[Proposition 2]{zhang2022safe}. We omit the proof due to space constraint. 
We note that the class of SNCBFs is a special subset of SCBFs in Proposition \ref{prop:verify_scbf}. In the following, we introduce the concept of valid SNCBFs, and present how to synthesize them. 
Based on Proposition \ref{prop:verify_scbf} and Definition \ref{def:feasibility}, feasible SCBFs can be defined as follows. 

\begin{definition}[Feasible SNCBF]
\label{def:feasibility_scbf}
    The SNCBF $b$ is feasible if and only if $\forall \hat{x}\in \mathcal{D}^{\gamma}$, $\exists u$ s.t. $\xi(\hat{x}) + \frac{\partial b}{\partial x}g(\hat{x})u\geq -\hat{b}^{\gamma}(\hat{x})$. 
\end{definition}

Besides the feasibility property given in Definition \ref{def:feasibility_scbf}, a valid SNCBF also needs to be correct as shown in Definition \ref{def:correctness}. However, we note that there may exist infinitely many valid SNCBFs, making the synthesis of valid SNCBFs computationally expensive. In this work, we focus on synthesizing valid SNCBFs that encompass the largest possible safety region. To this end, we define an operator $Vol(\mathcal{D}^\gamma)$ to represent the volume of the set $\mathcal{D}^{\gamma}$, and synthesize a valid SNCBF such that $Vol(\mathcal{D}^\gamma)$ is maximized. 
% A valid SNCBF is feasible as defined in Definition \ref{def:feasibility_scbf} and is correct defined in Definition \ref{def:correctness}. 
% Besides, a good SNCBF should not only be valid but also cover as much safe region as possible. We define an operator $Vol(\mathcal{D}_\gamma)$ represent the volume of the set $\mathcal{D}^{\gamma}$.  We next demonstrate how to synthesize a valid SNCBF. 
% To ensure the synthesized SCBF, we proposed the following loss function
% loss function design goes here

We denote the training dataset as $\mathcal{T}:=\{\hat{x}_{1}, \dots \hat{x}_{N}\mid \hat{x}_{i}
\in \mathcal{X} \quad \forall i \}$, where $N$ is the number of samples. The dataset $\mathcal{T}$ is generated by simulating estimates with fixed point sampling summarized in \cite{dawson2023safe}. We first uniformly discretize the state space into cells with length vector $L$. Next, we uniformly sample fixed points $x_{f}$ from the state space $\mathcal{X}$. Then we simulate the estimates by introduce perturbed with a small uniform noise $\rho[j]$ over interval $[x_{f}[j]-0.5 L[j], x_{f}[j]+0.5 L[j]]$. Finally, we have the sampling data $\hat{x}=x_{f}+\rho\in \mathcal{T}\subseteq \mathcal{X}$.
% The estimates $x_{R}$ are synthesized with $x_{f}$ perturbed by Gaussian noise, i.e., $x_{R}[j] = x_{f}[j] + \mathcal{N}(0, \sigma_{j}^2)$ where $\sigma_{j}$ is the standard deviation of corresponding sensor indexed $j$.

Then a valid SNCBF can be trained using $\mathcal{T}$ by solving the following optimization program. 
%The training of SNCBF can be summarized as a constrained optimization problem as follows. 
\begin{align}
    \label{eq:train_obj}
    \max_{\theta}&\quad{Vol(\mathcal{D}^\gamma)} \\
    \label{eq:train_feasible_cons}
    s.t. & \quad \xi(\hat{x}) \geq 0 \quad \forall \hat{x}\in \partial \mathcal{D}^{\gamma} \\
    \label{eq:train_correct_cons}
    & \quad \hat{b}_{\theta}(\hat{x}) \leq h(\hat{x}) \quad \forall \hat{x}\in \mathcal{X}\backslash\mathcal{D}^{\gamma}
\end{align}
where $\mathcal{D}^\gamma:=\{\hat{x}\mid \hat{b}^{\gamma}_{\theta}(\hat{x})\geq 0\}$. 
Solving the constrained optimization problem is challenging. In this work, we convert the constrained optimization to an unconstrained one using the Lagrangian method \cite{hestenes1969multiplier}, which introduces a Lagrangian multiplier to penalize violations of constraints. The unconstrained optimization problem is formulated as follows. 
\begin{equation}
    \label{eq:uncons_opt}
    \min_{\theta}\quad{-Vol(\mathcal{D}_{\theta}^{\gamma})} + \lambda_{f}\mathcal{L}_f + \lambda_{c}\mathcal{L}_c 
\end{equation}
where $\mathcal{L}_f$ is the loss for feasibility violation to replace the constraint \eqref{eq:train_feasible_cons}, $\mathcal{L}_f$ represents correctness loss for the constraint \eqref{eq:train_correct_cons}, and $\lambda_{f}$ and $\lambda_{c}$ are Lagrangian multiplier for feasibility loss and correctness loss, respectively. 
The objective function \eqref{eq:train_obj} is converted to the following quantity
\begin{equation}
    \label{eq:volume_obj}
    Vol(\mathcal{D}_{\theta}^{\gamma}) = \sum_{\hat{x}\in \mathcal{T}}{-ReLU(h(\hat{x}))ReLU(-b_{\theta}(\hat{x}))}. 
\end{equation}
The idea is to penalize for the points $\hat{x}$ in safety region, i.e., $h(\hat{x})>0$ but being regarded as unsafe, i.e., $b_{\theta}(\hat{x})<0$. 
The penalty of feasibility constraint \eqref{eq:train_feasible_cons} is defined as
\begin{equation}
    \mathcal{L}_f = \sum_{\hat{x}\in \mathcal{T}} -\Delta(\hat{x}) ReLU(-\xi(\hat{x}) - \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u) 
\end{equation}
where $\Delta(\hat{x})$ is an indicate function where $\Delta(\hat{x}):= 1$ if $b_{\theta}(\hat{x})=\overline{b}^{\gamma}$ or $\Delta(\hat{x}):= 0$ otherwise. The function $\Delta$ is designed to pick points $\hat{x}$ s.t. $b_{\theta}(\hat{x})=0$. We penalize for the points that the following two condition hold. 
\begin{enumerate}
    \item $b_{\theta}(\hat{x})=0$.
    \item $\xi(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u <0 $. 
\end{enumerate}
The control input $u$ is computed by a minimum effort controller as follows. 
\begin{equation}
\begin{split}
    \min_{u} & \quad u^{T}u \\
    s.t. & \quad \xi(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u \geq -\hat{b}_{\theta}(\hat{x})
\end{split}
\end{equation}
Similarly, the correctness constraint \eqref{eq:train_correct_cons} is defined as 
\begin{equation}
    \label{eq:correctness_loss}
    \mathcal{L}_c = \sum_{x\in \mathcal{T}}{ReLU(-h(\hat{x}))ReLU(b_{\theta}(\hat{x}))}
\end{equation}
The loss function for correctness constraint is design to penalize for the points $\hat{x}$ outside of the safety region, i.e., $h(\hat{x})<0$ but being regarded as safe, i.e., $b_{\theta}(\hat{x})>0$. 
When $\mathcal{L}_c$ and $\mathcal{L}_f$ converge to $0$, the trained $b_{\theta}$ is a good SNCBF candidate. 
% The proposed framework can either train a bank of SNCBF or a solo SNCBF that can further be used for safety constraint construction. 


\subsection{Synthesis of FT-SNCBF}
% Synthesis of FT-SNCBF 
% Fault-tolerent is an extension of SNCBF
% conclude what we have in previous section and introduce what we are going to have in this section
In the previous subsection, we have the feasibility and correctness properties for SNCBFs and the training procedure. In this subsection, we first extend these two properties for adversarial scenario. Specifically, we want a function $b_{\theta}$ to satisfy properties defined in Definition \ref{def:feasibility_scbf} and Definition \ref{def:correctness}. Based on the derived properties, we next formulate the loss function to train a valid FT-SNCBF for all fault pattern.

Define \begin{equation*}
\overline{b}_{\theta}^{\gamma_{i}}
= \sup_{x,x^{0}}{\left\{b_{\theta}(\hat{x}) : ||x-x^{0}||_{2} \leq \gamma_{i}\right.} \\
\left. \text{ and } \hat{b}_{\theta}(x^{0})=0\right\}
\end{equation*}
The following proposition gives the  necessary and sufficient condition for a function $b_{\theta}$ to be a FT-SNCBF.  

\begin{proposition}
\label{prop:verify_ftscbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $b_{\theta}(\hat{x})$ is a FT-SNCBF if and only if there is no $\hat{x}\in \mathcal{D}^{\gamma_i}$, satisfying
$\frac{\partial b}{\partial x}g(\hat{x}) = 0$ , $\xi_{i}(\hat{x}) < 0$ for all $i\in Z_t$ where 
\begin{multline}
\label{eq:ftsncbf_cond}
    \xi_{i}(\hat{x}) =  \frac{\partial b}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x})K\nu\right) + \\
    ||\frac{\partial h}{\partial x}(\hat{x}_{t,i})K_{t,i}c||_{2} +  \hat{b}^{\gamma_i}(\hat{x}).
\end{multline}
and $\hat{b}_{\theta}^{\gamma_i}(\hat{x})=b_{\theta}(\hat{x})-\overline{b}^{\gamma}$
\end{proposition}
The proposition can be proved using the similar idea to Proposition \ref{prop:verify_scbf}. We omit the proof due to space limit. 

Similarly, we define the objective function as \eqref{eq:volume_obj} and the correctness constraint as \eqref{eq:correctness_loss}. The penalty of feasibility constraints \eqref{eq:train_feasible_cons} is defined as $\mathcal{L}_{f} = \sum_{i\in Z_t}{\mathcal{L}^{i}_{f}}$, where
\begin{equation*}
    \mathcal{L}^{i}_{f} = \sum_{\hat{x}\in \mathcal{T}} -\overline{\Delta}_{i}(\hat{x}) ReLU(-\xi_{i}(\hat{x}) - \frac{\partial b_{\theta}}{\partial x}(\hat{x}) u) 
\end{equation*}
where $\overline{\Delta}(\hat{x})$ is an indicate function where $\overline{\Delta}(\hat{x}):= 1$ if $b_{\theta}(\hat{x})=\max_{i\in Z_t}{\{\overline{b}^{\gamma_i}\}}$ or $\Delta(\hat{x}):= 0$ otherwise. The control input $u$ is computed by a minimum effort controller as follows. 
\begin{equation}
\label{eq:ctrl_multiSNCBF}
\begin{split}
    \min_{u} & \quad u^{T}u \\
    s.t. & \quad \xi_{i}(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}(\hat{x}) u \geq -\hat{b}_{\theta}(\hat{x}) \quad \forall i\in Z_t
\end{split}
\end{equation}
When $\mathcal{L}_c$ and all $\mathcal{L}_f$ converge to $0$, the trained $b_{\theta}$ is a good SNCBF candidate. Note that a good SNCBF candidate does not guarantee valid. The verification of a SNCBF candidate is needed and is a non-trivial process. 

\subsection{Fault Tolerant Framework}
% FT-Framework (Controller synthesis)
% EKF banks FT-framework
% Safety guarantee
A training procedure is proposed in previous sections for SNCBF and FT-SNCBF. However, to ensure safety of a system, a fault-tolerant framework for safe control in non-trivial. Hence, in this section, we address this issue. 
Since we do not know the fault pattern $r$, we construct estimators excluding faulty sensors by maintaining $m$ EKFs. Each EKF corresponds to a different possible fault pattern in $\{r_1,\dots r_m\}$. We ensure safety with probability $(1-\epsilon)$ by synthesizing one SNCBF and construct $m+1$ SNCBF constraints for each fault pattern on the control input. The deployment of the proposed FT-Framework can be summarized in the following Algorithm.
\begin{algorithm}[h]
\begin{algorithmic}[]
\caption{Fault-Tolerant Safe Control}
    \State \textbf{Input:} Sensor Input $y_{t}$, known fault pattern $\mathcal{F}$, trained FT-SNCBF $b_{\theta}$
    \State \textbf{Output:} Control Input $u$
    \Procedure{$u = FTC$}{$y_{t}\mid \mathcal{F}, b_{\theta}$}
    \State $\hat{x}_{t,0} \leftarrow EKF(y_{t,0})$.
    \For{$i,j \in \{1,\dots,m\}$ and $i\neq j$}
        \State $\hat{x}_{t,i} \leftarrow EKF(y_{t,i})$.
        \State $\hat{x}_{t,i,j} \leftarrow EKF(y_{t,i,j})$.
    \EndFor
    \State $Z_{t} \leftarrow \{1, \dots, m\}$. 
    \State Search for $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$ by solving \eqref{eq:ctrl_multiSNCBF}. 
    \Comment{Step 1}
    \If{No such $u_{t}$ can be found}
    \Comment{Step 2}
    \For{$i,j \in Z_t$ s.t. $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} > \theta_{ij}$} 
        \If{$||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} > \theta_{ij}/2$}
            \State $Z_{t} \leftarrow Z_{t} \setminus \{i\}$
        \Else
            \State $Z_{t} \leftarrow Z_{t} \setminus \{j\}$
        \EndIf
        \If{$\bigcap_{i \in Z_{t}}{\Omega_{i}} \neq \emptyset$}
            \State Search for $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$ by solving \eqref{eq:ctrl_multiSNCBF}. 
        \EndIf
    \EndFor
    \If{No such $u_{t}$ can be found}
        \Comment{Step 3}
        \State $i_{r} \leftarrow \min_{i}{\{\overline{y}_{t,i}-\overline{c}_{i}\hat{x}_{t,i}\}}$. 
        \State $Z_{t} \leftarrow \{i_{r}\}$.
        \State Search for $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$ by solving \eqref{eq:ctrl_multiSNCBF}. 
    \EndIf
    \EndIf
    \State \Return{$u_{t}$}
    \EndProcedure
\end{algorithmic}
\label{alg:ftcontrol}
\end{algorithm}

We next show the safety guarantee of the system under sensor faults. 
\begin{theorem}[Safety Guarantee under Sensor Faults]
    \label{th:FT_Safety}
    Given a well-trained FT-SNCBF $b_{\theta}$ s.t. the conditions in Proposition \ref{prop:verify_ftscbf} are satisfied for $i\in Z_{t}$.  
    Suppose  $\gamma_{1},\ldots,\gamma_{m}$, and $\theta_{ij}$ for $i < j$ are chosen such that the following conditions are satisfied:
    \begin{enumerate}
    \item Define  $\Lambda_{i}(\hat{x}_{t,i}) = \frac{\partial h_{i}}{\partial x}(\hat{x}_{t,i})g(\hat{x}_{t,i})$. There exists $\delta > 0$ such that for any $X_{t}^{\prime} \subseteq X_{t}(\delta)$ satisfying $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} \leq \theta_{ij}$ for all $i,j \in X_{t}^{\prime}$,  there exists $u$ such that
    \begin{equation}
    \label{eq:FT-CBF2}
    \Lambda_{i}(\hat{x}_{t,i})u > \xi_{i}(\hat{x})
    \end{equation}
    for all $i \in Z_{t}$.
    \item For each $i$, when $r=r_{i}$, 
    \begin{multline}
    \label{eq:FT-CBF3}
    Pr(||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \theta_{ij}/2 \ \forall j, ||\hat{x}_{t,i}-x_{t}||_{2} \leq \gamma_{i} \ \forall t)\\
     \geq 1-\epsilon.
    \end{multline}
    \end{enumerate}
    Then $Pr(x_{t} \in \mathcal{D} \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$.
\end{theorem}
\begin{proof}
    By Proposition \ref{prop:verify_ftscbf}, there exist $u_t$ s.t. \eqref{eq:ftsncbf_cond} hold for all $\hat{x}\in \mathcal{D}_{\theta}^{\gamma_i}\quad \forall i\in Z_{t}$. By \cite[Theorem 3]{clark2020control} we have that $\Omega_{i}$ holds 
    $\forall \hat{x}\in \mathcal{D}^{\gamma}_{\theta}$ $\forall i\in Z_{t}$. Therefore, by Theorem \ref{theorem:SCBF}, 
    \begin{multline*}
    Pr(x_{t} \in \mathcal{D} \ \forall t | ||\hat{x}_{t,i}-\hat{x}_{t}||_{2} \leq \gamma_{i}, \\ ||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \theta_{ij}/2 \ \forall t) 
    = 1
    \end{multline*}
    and $Pr(x_{t} \in \mathcal{D}\subseteq \mathcal{C} \ \forall t) > 1-\epsilon$ by (\ref{eq:FT-CBF3}).
\end{proof} 

% \subsection{FT-NCBF Design}
% The network is designed to take all estimates $\hat{x}_i$, $\forall i$ and indicator $I$. Intuitively, the indicator works like a mask to filter out unwanted estimates and activate different gain for corresponding $\gamma_i$

% \subsection{EKF Residual-based Fault Pattern Classification (Potential)}
% \textbf{Action needed **} The classification requires us to derive a guarantee. Fundamentally, the classifier is to make the whole design of the framework more cohesive by removing step 1, 2 and 3. 


==> sections/FTNCBF.tex <==
\section{Fault Tolerant NCBF}\label{sec:sol}
% In this section we present the stochastic NCBFs (SNCBFs) and fault-tolerant SNCBFs (FT-SNCBFs). 
In this section, we first give some background including the Extended Kalman Filter (EKF) and Stochastic CBFs (SCBFs). We next present an overview of the proposed method. Then, we demonstrate the theoretical foundation of SNCBFs and FT-SNCBFs. With the theories support, we present the training process and formulation fault-tolerant framework when deploying

% Background
% EKF
% SCBF
% FT-framework

% High level intuition
% (make sure that the details of overview will be coverd in the later subsections or can be found in other references)

% Synthesis of SNCBF (Training)
% theoretical foundation provide the criterion on what are good SNCBFs
% - correctness (how to check)
% - feasibility (derive condition for SNCBF feasibility)
% Training (Loss function design)
% Based on theroetical foundation, we design the loss function to guide SNCBF to converge

% Synthesis of FT-SNCBF 
% Fault-tolerent is an extension of SNCBF

% FT-Framework (Controller synthesis)
% EKF banks FT-framework
% Safety guarantee

\subsection{Background}
\subsubsection{Extended Kalman Filter}
\begin{assumption}
\label{assumption:ekf}
The SDEs (\ref{eq:state-sde}) and (\ref{eq:output-sde}) satisfy the conditions:
\begin{enumerate}
\item There exist constants $\beta_{1}$ and $\beta_{2}$ such that $\mathbf{E}(\sigma_{t}\sigma_{t}^{T}) \geq \beta_{1} I$ and $\mathbf{E}(\nu_{t}\nu_{t}^{T}) \geq \beta_{2} I$ for all $t$. 
\item The pair $[\frac{\partial \overline{f}}{\partial x}(x,u),c]$ is uniformly detectable.
% \item The system has $(p-1)$ redundancy, where $p>1$. 
\item Let $\phi$ be defined by $$\overline{f}(x,u)-\overline{f}(\hat{x},u) = \frac{\partial \overline{f}}{\partial x}(x - \hat{x}) + \phi(x,\hat{x},u).$$ Then there exist real numbers $k_{\phi}$ and $\epsilon_{\phi}$ such that $$||\phi(x,\hat{x},u)|| \leq k_{\phi}||x-\hat{x}||_{2}^{2}$$ for all $x$ and $\hat{x}$ satisfying $||x-\hat{x}||_{2} \leq \epsilon_{\phi}$. 
\end{enumerate}
\end{assumption} 

\begin{theorem}[\cite{reif2000stochastic}]
\label{theorem:EKF}
Suppose that the conditions of Assumption \ref{assumption:ekf} hold. Then there exists $\delta > 0$ such that $\sigma_{t}\sigma_{t}^{T} \leq \delta I$ and $\nu_{t}\nu_{t}^{T} \leq \delta I$. For any $0<\epsilon <1$, there exists $\gamma > 0$ such that $$Pr\left(\sup_{t \geq 0}{||x_{t}-\hat{x}_{t}||_{2} \leq \gamma}\right) \geq 1-\epsilon.$$ 
\end{theorem}

\subsubsection{Stochastic CBFs}
\begin{theorem}[\cite{clark2020control}]
\label{theorem:SCBF}
    For a system (\ref{eq:state-sde})--(\ref{eq:output-sde}) with safety region defined by (\ref{eq:safe-region}), define
    $$\overline{b}^{\gamma} = \sup_{x,x^{0}}{\{b(\hat{x}) : ||x-x^{0}||_{2} \leq \gamma \text{ and } b(x^{0})=0\}}. $$
    Let $\hat{b}(\hat{x}) := b(\hat{x})-\overline{b}^{\gamma}$. Let $\hat{x}_{t}$ denote the EKF estimate of $x_{t}$, and suppose that there exists a constant $\delta > 0$ such that   
    whenever $\hat{b}(\hat{x}_{t}) < \delta$, $u_{t}$ is chosen to satisfy
    \begin{multline}
    \label{eq:SCBF-2}
    \frac{\partial b}{\partial x}(\hat{x}_{t})\overline{f}(\hat{x}_{t},u_{t}) - \gamma||\frac{\partial b}{\partial x}(\hat{x}_{t})K_{t}c||_{2} \\
    + \frac{1}{2}\mathbf{tr}\left(\nu_{t}^{T}K_{t}^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x}_{t})K_{t}\nu_{t}\right) \geq -\hat{b}(\hat{x}_{t}).
    \end{multline}
    Then $Pr(x_{t} \in \mathcal{D} \ \forall t | \ ||x_{t}-\hat{x}_{t}||_{2} \leq \gamma \ \forall t) = 1$. 
\end{theorem}

% The proof of Theorem \ref{theorem:SCBF} is very similar to the proof of Theorem 7 from \cite{clark2021control} and is omitted due to space constraints.
Intuitively,  Eq. (\ref{eq:SCBF-2}) implies that as the state approaches the boundary, the control input is chosen such that the rate of increase of the barrier function decreases to zero. Hence Theorem \ref{theorem:SCBF} implies that if there exists an SCBF for a system, then the safety condition is satisfied with probability $(1-\epsilon)$ when an EKF is used as an estimator and the control input is chosen at each time $t$ to satisfy (\ref{eq:SCBF-2}).

\begin{definition}[SCBF]
\label{Def:SCBF}
    The function $h$ is a \emph{Stochastic Control Barrier Function (SCBF)} of the system, if for all $\hat{x}_t$ satisfying $h(\hat{x}_t)>0$ there exists $u_t$ s.t. $\forall z_t$ with $\|z_t\|\leq \gamma$ \eqref{eq:SCBF-2} is satisfied. 
\end{definition}

\subsection{Overview}
% High level intuition
% (make sure that the details of overview will be coverd in the later subsections or can be found in other references)
Our goal is to synthesize a NCBF to play the role of SCBFs. To let one NCBF to replace the SCBFs corresponding to all possible fault patterns, we want to introduce the reasoning component as an input. The reasoning input belongs to a discrete space, indicating the fault patterns $I\in \mathcal{I}$, where $\mathcal{I}$ is the set of all possible fault patterns. To verify the FT-NCBF we verify $b_{\theta}(x\mid I)$, $\forall I\in \mathcal{I}$ where $I$ is the discrete input of fault patterns. In what follows, we will demonstrate our design of the pipeline. 


\subsection{Synthesis of SNCBF}
% Synthesis of SNCBF (Training)
% theoretical foundation provide the criterion on what are good SNCBFs
% - correctness (how to check)
% - feasibility (derive condition for SNCBF feasibility)
% Training (Loss function design)
% Based on theroetical foundation, we design the loss function to guide SNCBF to converge

% We generate with $b_{\theta}(x)$ with sensor noise and under different fault patterns. 

% Theorem to define a valid SCBF for polyCBF and NCBF
In what follows, we describe how to synthesize stochastic neural CBFs (SNCBFs). We first introduce the SCBFs, among which SNCBFs constitute a special class represented by neural networks. 
% The safety of a stochastic system can be ensured safe by Theorem \ref{theorem:SCBF} given a function $b(x)$. In what follows, we shows criterion for SCBF candidates. 
% Let the estimation error to be represented as $z_t = (x_t-\hat{x}_t)$. 
The following proposition gives the  necessary and sufficient conditions for a function $b$ to be a SCBF.  
\begin{proposition}
\label{prop:verify_scbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $b(\hat{x})$ is a SCBF if and only if there is no $\hat{x}\in \mathcal{D}^{\gamma}:=\{\hat{x}\mid \hat{b}^{\gamma}(\hat{x})\geq 0\}$, satisfying
$\frac{\partial b}{\partial x}g(\hat{x}) = 0$ and $\xi(\hat{x}) < 0$, where 
\begin{multline}
\label{eq:prop2cond}
    \xi(\hat{x}) =  \frac{\partial b}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x})K\nu\right) + \\
    ||\frac{\partial b}{\partial x}(\hat{x})K_{t,i}c||_{2} +  \hat{b}(\hat{x}).
\end{multline}
\end{proposition}
The proposition is derived based on \cite[Proposition 2]{zhang2022safe}. We omit the proof due to space constraint. 
We note that the class of SNCBFs is a special subset of SCBFs in Proposition \ref{prop:verify_scbf}. In the following, we introduce the concept of valid SNCBFs, and present how to synthesize them. 
Based on Proposition \ref{prop:verify_scbf} and Definition \ref{def:feasibility}, feasible SNCBFs can be defined as follows. 

\begin{definition}[Feasible SNCBF]
\label{def:feasibility_scbf}
    The SNCBF $b$ is feasible if and only if $\forall \hat{x}\in \mathcal{D}^{\gamma}$, $\exists u$ s.t. $\xi(\hat{x}) + \frac{\partial b}{\partial x}g(\hat{x})u\geq 0$. 
\end{definition}

Besides the feasibility property given in Definition \ref{def:feasibility_scbf}, a valid SNCBF also needs to be correct as shown in Definition \ref{def:correctness}. However, we note that there may exist infinitely many valid SNCBFs, making the synthesis of valid SNCBFs computationally expensive. In this work, we focus on synthesizing valid SNCBFs that encompass the largest possible safety region. To this end, we define an operator $Vol(\mathcal{D}^\gamma)$ to represent the volume of the set $\mathcal{D}^{\gamma}$, and synthesize a valid SNCBF such that $Vol(\mathcal{D}^\gamma)$ is maximized. 
% A valid SNCBF is feasible as defined in Definition \ref{def:feasibility_scbf} and is correct defined in Definition \ref{def:correctness}. 
% Besides, a good SNCBF should not only be valid but also cover as much safe region as possible. We define an operator $Vol(\mathcal{D}_\gamma)$ represent the volume of the set $\mathcal{D}^{\gamma}$.  We next demonstrate how to synthesize a valid SNCBF. 
% To ensure the synthesized SCBF, we proposed the following loss function
% loss function design goes here

We denote the training dataset as $\mathcal{T}:=\{\hat{x}_{1}, \ldots, \hat{x}_{N}\mid \hat{x}_{i}
\in \mathcal{X}, \forall i =1,\ldots,N\}$, where $N$ is the number of samples. The dataset $\mathcal{T}$ is generated by simulating estimates with fixed point sampling summarized in \cite{dawson2023safe}. We first uniformly discretize the state space into cells with length vector $L$. Next, we uniformly sample the center of discretized cell as fixed points $x_{f}$. Then we simulate the estimates by introducing a perturbation $\rho[j]$  sampled uniformly from interval $[x_{f}[j]-0.5 L[j], x_{f}[j]+0.5 L[j]]$. Finally, we have the sampling data $\hat{x}=x_{f}+\rho\in \mathcal{T}\subseteq \mathcal{X}$.
% The estimates $x_{R}$ are synthesized with $x_{f}$ perturbed by Gaussian noise, i.e., $x_{R}[j] = x_{f}[j] + \mathcal{N}(0, \sigma_{j}^2)$ where $\sigma_{j}$ is the standard deviation of corresponding sensor indexed $j$.

Then a valid SNCBF can be trained using $\mathcal{T}$ by solving the following optimization program. 
%The training of SNCBF can be summarized as a constrained optimization problem as follows. 
\begin{align}
    \label{eq:train_obj}
    \max_{\theta}&\quad{Vol(\mathcal{D}^\gamma)} \\
    \label{eq:train_feasible_cons}
    s.t. & \quad \xi(\hat{x}) \geq 0 \quad \forall \hat{x}\in \partial \mathcal{D}^{\gamma} \\
    \label{eq:train_correct_cons}
    & \quad \hat{b}_{\theta}(\hat{x}) \leq h(\hat{x}) \quad \forall \hat{x}\in \mathcal{X}\backslash\mathcal{D}^{\gamma}
\end{align}
where $\mathcal{D}^\gamma:=\{\hat{x}\mid \hat{b}^{\gamma}_{\theta}(\hat{x})\geq 0\}$. 
Solving the constrained optimization problem is challenging. In this work, we convert the constrained optimization to an unconstrained one using the Lagrangian method \cite{hestenes1969multiplier}, which introduces a Lagrangian multiplier to penalize violations of the constraints. The unconstrained optimization problem is formulated as follows. 
\begin{equation}
    \label{eq:uncons_opt}
    \min_{\theta}\quad{-Vol(\mathcal{D}_{\theta}^{\gamma})} + \lambda_{f}\mathcal{L}_f + \lambda_{c}\mathcal{L}_c 
\end{equation}
where $\mathcal{L}_f$ is the loss for feasibility violation corresponding to constraint \eqref{eq:train_feasible_cons}, $\mathcal{L}_f$ represents correctness loss for constraint \eqref{eq:train_correct_cons}, and $\lambda_{f}$ and $\lambda_{c}$ are Lagrangian multipliers for feasibility loss and correctness loss, respectively. 
The objective function \eqref{eq:train_obj} is approximated by the following quantity
\begin{equation}
    \label{eq:volume_obj}
    Vol(\mathcal{D}_{\theta}^{\gamma}) = \sum_{\hat{x}\in \mathcal{T}}{-ReLU(h(\hat{x}))ReLU(-b_{\theta}(\hat{x}))}. 
\end{equation}
The idea is to penalize for the points $\hat{x}$ in safety region but not in $\mathcal{D}^\gamma$, i.e., $h(\hat{x})>0$ but being regarded as unsafe, i.e., $b_{\theta}(\hat{x})<0$. 
The penalty of feasibility constraint \eqref{eq:train_feasible_cons} is defined as
\begin{equation}
    \mathcal{L}_f = \sum_{\hat{x}\in \mathcal{T}} -\Delta(\hat{x}) ReLU(-\xi(\hat{x}) - \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u + \hat{b}(\hat{x})) 
\end{equation}
where $\Delta(\hat{x})$ is an indicate function where $\Delta(\hat{x}):= 1$ if $b_{\theta}(\hat{x})=\overline{b}^{\gamma}$ or $\Delta(\hat{x}):= 0$ otherwise. The function $\Delta$ is designed to pick points $\hat{x}$ s.t. $b_{\theta}(\hat{x})=0$. We penalize for the points that the following two condition hold
\begin{enumerate}
    \item $b_{\theta}(\hat{x})=0$.
    \item $\xi(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u <0 $. 
\end{enumerate}
The control input $u$ is computed by a minimum effort controller as follows. 
\begin{equation}
\begin{split}
    \min_{u} & \quad u^{T}u \\
    s.t. & \quad \xi(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u \geq 0
\end{split}
\end{equation}
Similarly, the correctness constraint \eqref{eq:train_correct_cons} is defined as 
\begin{equation}
    \label{eq:correctness_loss}
    \mathcal{L}_c = \sum_{x\in \mathcal{T}}{ReLU(-h(\hat{x}))ReLU(b_{\theta}(\hat{x}))}
\end{equation}
The loss function for correctness constraint is design to penalize for the points $\hat{x}$ outside of the safety region, i.e., $h(\hat{x})<0$ but being regarded as safe, i.e., $b_{\theta}(\hat{x})>0$. 
When $\mathcal{L}_c$ and $\mathcal{L}_f$ converge to $0$, the trained $b_{\theta}$ is a good SNCBF candidate. 
% The proposed framework can either train a bank of SNCBF or a solo SNCBF that can further be used for safety constraint construction. 


\subsection{Synthesis of FT-SNCBF}
% Synthesis of FT-SNCBF 
% Fault-tolerent is an extension of SNCBF
% conclude what we have in previous section and introduce what we are going to have in this section
In the previous subsection, we introduced the feasibility and correctness properties for SNCBFs and the training procedure. In this subsection, we first generalize the feasibility and correctness properties to the adversarial scenario. Specifically, we desire a function $b_{\theta}$ to satisfy the properties defined in Definition \ref{def:feasibility_scbf} and \ref{def:correctness}. Based on the generalized properties, we next formulate a loss function to train a valid fault tolerant-SNCBF (FT-SNCBF) for all fault patterns.

Define \begin{equation*}
\overline{b}_{\theta}^{\gamma_{i}}
= \sup_{x,x^{0}}{\left\{b_{\theta}(\hat{x}) : ||x-x^{0}||_{2} \leq \gamma_{i}\right.} \\
\left. \text{ and } \hat{b}_{\theta}(x^{0})=0\right\}.
\end{equation*}
The following proposition gives the  necessary and sufficient conditions for a function $b_{\theta}$ to be a FT-SNCBF.  

\begin{proposition}
\label{prop:verify_ftscbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $b_{\theta}(\hat{x})$ is a FT-SNCBF if and only if there is no $\hat{x}\in \mathcal{D}^{\gamma_i}$, satisfying
$\frac{\partial b}{\partial x}g(\hat{x}) = 0$ , $\xi_{i}(\hat{x}) < 0$ for all $i\in Z_t$ where 
\begin{multline}
\label{eq:ftsncbf_cond}
    \xi_{i}(\hat{x}) =  \frac{\partial b}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x})K\nu\right) + \\
    ||\frac{\partial h}{\partial x}(\hat{x})K_{t,i}c||_{2} +  \hat{b}^{\gamma_i}(\hat{x}).
\end{multline}
and $\hat{b}_{\theta}^{\gamma_i}(\hat{x})=b_{\theta}(\hat{x})-\overline{b}^{\gamma}$
\end{proposition}
The proposition can be proved using the similar idea to Proposition \ref{prop:verify_scbf}. We omit the proof due to space limit. 

Similarly, we define the unconstrained objective function for FT-SNCBF training as 
\begin{equation}
    \label{eq:train_ftsncbf}
    \min_{\theta}\quad{-Vol(\mathcal{D}_{\theta}^{\gamma})} + \sum_{i\in Z_t}{\mathcal{L}^{i}_{f}} + \mathcal{L}_c. 
\end{equation}
We define the objective function as \eqref{eq:volume_obj} and the correctness constraint as \eqref{eq:correctness_loss}. The penalty of feasibility constraints \eqref{eq:train_feasible_cons} is defined as $\mathcal{L}_{f} = \sum_{i\in Z_t}{\mathcal{L}^{i}_{f}}$, where
\begin{equation*}
    \mathcal{L}^{i}_{f} = \sum_{\hat{x}\in \mathcal{T}} -\overline{\Delta}_{i}(\hat{x}) ReLU(-\xi_{i}(\hat{x}) - \frac{\partial b_{\theta}}{\partial x}(\hat{x}) u + \hat{b}^{\gamma_i}(\hat{x})) 
\end{equation*}
where $\overline{\Delta}(\hat{x})$ is an indicate function where $\overline{\Delta}(\hat{x}):= 1$ if $b_{\theta}(\hat{x})\leq\max_{i\in Z_t}{\{\overline{b}^{\gamma_i}\}}$ or $\Delta(\hat{x}):= 0$ otherwise. The control input $u$ is computed by a minimum effort controller as follows. 
\begin{equation}
\label{eq:ctrl_multiSNCBF}
\begin{split}
    \min_{u} & \quad u^{T}u \\
    s.t. & \quad \xi_{i}(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}(\hat{x}) u \geq 0 \quad \forall i\in Z_t
\end{split}
\end{equation}
When $\mathcal{L}_c$ and all $\mathcal{L}_f$ converge to $0$, the trained $b_{\theta}$ is a good SNCBF candidate. Note that a good SNCBF candidate does not guarantee valid. The verification of a SNCBF candidate is needed and is a non-trivial process. 

\subsection{Fault Tolerant Framework}
% FT-Framework (Controller synthesis)
% EKF banks FT-framework
% Safety guarantee
% A training procedure is proposed in previous sections for SNCBF and FT-SNCBF. However, to ensure safety of a system, a fault-tolerant framework for safe control in non-trivial. Hence, we address this issue in this subsection. 

In this subsection, we develop a fault tolerant framework which utilizes the learned FT-SNCBF to synthesize a control policy to guarantee safety.
We maintain $1+m+{m \choose 2}$ EKFs.
\begin{enumerate}
    \item $1$: One EKF is designed for fault free case. 
    \item $m$: Each EKF corresponds to a different possible fault pattern in $\{r_1,\dots r_m\}$. 
    \item ${m \choose 2}$: Each EKF corresponds to the combination of fault pattern $i,j\in\{r_1,\dots r_m\}$, $i\neq j$. 
\end{enumerate}
We ensure safety with probability $(1-\epsilon)$ by synthesizing a FT-SNCBF and construct $m+1$ corresponding constraints for each fault pattern on the control input. The deployment of the proposed FT-Framework can be summarized in the following Algorithm.
\begin{algorithm}[h]
\begin{algorithmic}[]
\caption{Fault-Tolerant Safe Control}
    \State \textbf{Input:} Sensor Input $y_{t}$, known fault pattern $\mathcal{F}$, trained FT-SNCBF $b_{\theta}$
    \State \textbf{Output:} Control Input $u$
    \Procedure{$u = FTC$}{$y_{t}\mid \mathcal{F}, b_{\theta}$}
    \State $\hat{x}_{t,0} \leftarrow EKF(y_{t,0})$.
    \For{$i,j \in \{1,\dots,m\}$ and $i\neq j$}
        \State $\hat{x}_{t,i} \leftarrow EKF(y_{t,i})$.
        \State $\hat{x}_{t,i,j} \leftarrow EKF(y_{t,i,j})$.
    \EndFor
    \State $Z_{t} \leftarrow \{1, \dots, m\}$. 
    \State Search for $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$ by solving \eqref{eq:ctrl_multiSNCBF}. 
    \Comment{Step 1}
    \If{No such $u_{t}$ can be found}
    \Comment{Step 2}
    \For{$i,j \in Z_t$ s.t. $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} > \theta_{ij}$} 
        \If{$||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} > \theta_{ij}/2$}
            \State $Z_{t} \leftarrow Z_{t} \setminus \{i\}$
        \Else
            \State $Z_{t} \leftarrow Z_{t} \setminus \{j\}$
        \EndIf
        \If{$\bigcap_{i \in Z_{t}}{\Omega_{i}} \neq \emptyset$}
            \State Search for $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$ by solving \eqref{eq:ctrl_multiSNCBF}. 
        \EndIf
    \EndFor
    \If{No such $u_{t}$ can be found}
        \Comment{Step 3}
        \State $i_{r} \leftarrow \min_{i}{\{\overline{y}_{t,i}-\overline{c}_{i}\hat{x}_{t,i}\}}$. 
        \State $Z_{t} \leftarrow \{i_{r}\}$.
        \State Search for $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$ by solving \eqref{eq:ctrl_multiSNCBF}. 
    \EndIf
    \EndIf
    \State \Return{$u_{t}$}
    \EndProcedure
\end{algorithmic}
\label{alg:ftcontrol}
\end{algorithm}

We next show the safety guarantee of the system under sensor faults. The following result gives sufficient conditions to guarantee safety. 
\begin{lemma}[\cite{clark2020control}]
    \label{lemma:ftsafe}
    Suppose  $\gamma_{1},\ldots,\gamma_{m}$, and $\theta_{ij}$ for $i < j$ are chosen such that the following conditions are satisfied:
    \begin{enumerate}
    \item Define  $\Lambda_{i}(\hat{x}_{t,i}) = \frac{\partial h_{i}}{\partial x}(\hat{x}_{t,i})g(\hat{x}_{t,i})$. There exists $\delta > 0$ such that for any $X_{t}^{\prime} \subseteq X_{t}(\delta)$ satisfying $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} \leq \theta_{ij}$ for all $i,j \in X_{t}^{\prime}$,  there exists $u$ such that
    \begin{equation}
    \label{eq:FT-CBF2}
    \Lambda_{i}(\hat{x}_{t,i})u > \xi_{i}(\hat{x})
    \end{equation}
    for all $i \in Z_{t}$.
    \item For each $i$, when $r=r_{i}$, 
    \begin{multline}
    \label{eq:FT-CBF3}
    Pr(||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \theta_{ij}/2 \ \forall j, ||\hat{x}_{t,i}-x_{t}||_{2} \leq \gamma_{i} \ \forall t)\\
     \geq 1-\epsilon.
    \end{multline}
    \end{enumerate}
    Then $Pr(x_{t} \in \mathcal{D} \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$.
\end{lemma}
However, Lemma \ref{lemma:ftsafe} depends on the existence of $u_{t}$. The following proposition provides sufficient condition of the existence of $u_{t}$ for all $\hat{x}\in \mathcal{D}^{\gamma_i}_{\theta}, \ \forall i\in Z_{t}$.  
\begin{proposition}
    \label{prop:u_f_ftsncbf}
    Suppose a FT-SNCBF $b_{\theta}$ satisfies the conditions in Proposition \ref{prop:verify_ftscbf} for $i\in Z_{t}$. Then, there always exists $u_{t}$ such that $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})u_{t}+\xi_{i}\geq 0$ $\forall \hat{x}\in \mathcal{D}_{\theta}^{\gamma_i}, \ \forall i\in Z_t$. 
\end{proposition}
\begin{proof}    
    We prove by showing there always exists $u_t$ such that \eqref{eq:SCBF-2} hold for two cases, namely, (i) $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})\neq0$ and (ii) $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})=0$. 
    For case (ii), we can always choose $u_{t}$ such that \eqref{eq:SCBF-2} holds for all $i\in Z_t$. For case (ii), there does not exist $\hat{x}$ such that $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})=0$ and $\xi_i(\hat{x})< 0$ by Proposition \ref{prop:verify_ftscbf}. Hence, $u_{t}$ can be any real value. 
\end{proof}
Finally, we present safety guarantee for system under sensor faults. 
\begin{theorem}[Safety Guarantee under Sensor Faults]
    \label{th:FT_Safety}
    Given a FT-SNCBF $b_{\theta}$ satisfies the conditions in Proposition \ref{prop:verify_ftscbf} for $i\in Z_{t}$. Suppose $\gamma_{1},\ldots,\gamma_{m}$, and $\theta_{ij}$ for $i < j$ are chosen such that conditions in \ref{lemma:ftsafe} hold. Then $Pr(x_{t} \in \mathcal{D} \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$. 
\end{theorem}
\begin{proof}
    By \cite[Theorem 3]{clark2020control} if there exist $u_{t}$ such that $\Omega_{i}$ holds 
    $\forall \hat{x}\in \mathcal{D}^{\gamma}_{\theta}$ $\forall i\in Z_{t}$ then, by Theorem \ref{theorem:SCBF}, 
    \begin{multline*}
    Pr(x_{t} \in \mathcal{D} \ \forall t | ||\hat{x}_{t,i}-\hat{x}_{t}||_{2} \leq \gamma_{i}, \\ ||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \theta_{ij}/2 \ \forall t) = 1
    \end{multline*}
    By Proposition \ref{prop:u_f_ftsncbf}, there exist $u_t$ s.t. $\Omega_{i}$ holds for all $\hat{x}\in \mathcal{D}^{\gamma_i}\quad \forall i\in Z_{t}$. 
    and $Pr(x_{t} \in \mathcal{D}\subseteq \mathcal{C} \ \forall t) > 1-\epsilon$ by (\ref{eq:FT-CBF3}).
\end{proof} 

% \subsection{FT-NCBF Design}
% The network is designed to take all estimates $\hat{x}_i$, $\forall i$ and indicator $I$. Intuitively, the indicator works like a mask to filter out unwanted estimates and activate different gain for corresponding $\gamma_i$

% \subsection{EKF Residual-based Fault Pattern Classification (Potential)}
% \textbf{Action needed **} The classification requires us to derive a guarantee. Fundamentally, the classifier is to make the whole design of the framework more cohesive by removing step 1, 2 and 3. 


==> sections/FTNCBF_v1.tex <==
% \section{Fault Tolerant NCBF}\label{sec:sol}
\section{Synthesis of Fault Tolerant SNCBF and Safety-Critical Control}\label{sec:sol}
% In this section we present the stochastic NCBFs (SNCBFs) and fault-tolerant SNCBFs (FT-SNCBFs). 
In this section, we first derive the necessary and sufficient conditions for stochastic neural control barrier functions (SNCBFs). 
We then generalize SNCBFs and propose fault tolerant SNCBFs (FT-SNCBFs).
We construct a loss function to learn FT-SNCBFs from data. 
We finally show how the learned FT-NCBFs can be used for the synthesis of control inputs to guarantee safety.

% Background
% EKF
% SCBF
% FT-framework

% High level intuition
% (make sure that the details of overview will be coverd in the later subsections or can be found in other references)

% Synthesis of SNCBF (Training)
% theoretical foundation provide the criterion on what are good SNCBFs
% - correctness (how to check)
% - feasibility (derive condition for SNCBF feasibility)
% Training (Loss function design)
% Based on theroetical foundation, we design the loss function to guide SNCBF to converge

% Synthesis of FT-SNCBF 
% Fault-tolerent is an extension of SNCBF

% FT-Framework (Controller synthesis)
% EKF banks FT-framework
% Safety guarantee


% \subsection{Roadmap of Solution Methodology}

% We first derive the necessary and sufficient conditions for a function to be a stochastic neural control barrier function (SNCBF).
% We then construct a loss function using the derived conditions to learn SNCBF from data.
% While SNCBFs can be used for safety-critical control synthesis of robotic systems in benign environments, we generalize them and propose fault tolerant SNCBFs (FT-SNCBFs) for systems under sensor faults and attacks.
% We present a data-driven method to learn FT-SNCBFs.
% Given the learned FT-SNCBFs, we formulate a quadratic program for the synthesis of control inputs to satisfy the safety constraint.
% Specifically, we maintain a set of EKFs, with each being associated with one fault pattern.


% \subsection{Overview}
% % High level intuition
% % (make sure that the details of overview will be coverd in the later subsections or can be found in other references)
% Our goal is to synthesize a NCBF to play the role of SCBFs. To let one NCBF to replace the SCBFs corresponding to all possible fault patterns, we want to introduce the reasoning component as an input. The reasoning input belongs to a discrete space, indicating the fault patterns $I\in \mathcal{I}$, where $\mathcal{I}$ is the set of all possible fault patterns. To verify the FT-NCBF we verify $b_{\theta}(x\mid I)$, $\forall I\in \mathcal{I}$ where $I$ is the discrete input of fault patterns. In what follows, we will demonstrate our design of the pipeline. 


\subsection{Synthesis of SNCBF}
% Synthesis of SNCBF (Training)
% theoretical foundation provide the criterion on what are good SNCBFs
% - correctness (how to check)
% - feasibility (derive condition for SNCBF feasibility)
% Training (Loss function design)
% Based on theroetical foundation, we design the loss function to guide SNCBF to converge

% We generate with $b_{\theta}(x)$ with sensor noise and under different fault patterns. 

% Theorem to define a valid SCBF for polyCBF and NCBF
In what follows, we describe how to synthesize SNCBFs. 
We first present the necessary and sufficient conditions for stochastic control barrier functions, among which SNCBFs constitute a special class represented by neural networks. 
% The safety of a stochastic system can be ensured safe by Theorem \ref{theorem:SCBF} given a function $b(x)$. In what follows, we shows criterion for SCBF candidates. 
% Let the estimation error to be represented as $z_t = (x_t-\hat{x}_t)$. 
% The following proposition gives the  necessary and sufficient conditions for a function $b$ to be a SCBF.  
\begin{proposition}
\label{prop:verify_scbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $b(\hat{x})$ is an SCBF if and only if there is no $\hat{x}\in \mathcal{D}^{\gamma}:=\{\hat{x}\mid \hat{b}(\hat{x})\geq 0\}$, satisfying
$\frac{\partial b}{\partial x}g(\hat{x}) = 0$ and $\xi(\hat{x}) < 0$, where 
\begin{multline}
\label{eq:prop2cond}
    \xi(\hat{x}) =  \frac{\partial b}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x})K\nu\right) + \\
    ||\frac{\partial b}{\partial x}(\hat{x})K_{t,i}c||_{2} +  \hat{b}(\hat{x}).
\end{multline}
\end{proposition}
The proposition is derived based on \cite[Proposition 2]{zhang2022safe}. We omit the proof due to space constraint. 
We note that the class of SNCBFs is a special subset of SCBFs in Proposition \ref{prop:verify_scbf}. In the following, we introduce the concept of valid SNCBFs, and present how to synthesize them. 
Based on Proposition \ref{prop:verify_scbf} and Definition \ref{def:feasibility}, feasible SNCBFs can be defined as follows. 

\begin{definition}[Feasible SNCBF]
\label{def:feasibility_scbf}
    The SNCBF $b_\theta$ parameterized by $\theta$ is feasible if and only if $\forall \hat{x}\in \mathcal{D}^{\gamma}$, $\exists u$ s.t. $\xi(\hat{x}) + \frac{\partial b_\theta}{\partial x}g(\hat{x})u\geq 0$. 
\end{definition}

Besides the feasibility property given in Definition \ref{def:feasibility_scbf}, a valid SNCBF $b_\theta$ also needs to be correct as shown in Definition \ref{def:correctness}. However, we note that there may exist infinitely many valid SNCBFs, making the synthesis of valid SNCBFs computationally expensive. In this work, we focus on synthesizing valid SNCBFs that encompass the largest possible safety region. To this end, we define an operator $Vol(\mathcal{D}^\gamma)$ to represent the volume of the set $\mathcal{D}^{\gamma}$, and synthesize a valid SNCBF such that $Vol(\mathcal{D}^\gamma)$ is maximized. The optimization program is given as follows
\begin{align}
    \label{eq:train_obj}
    \max_{\theta}&\quad{Vol(\mathcal{D}^\gamma)} \\
    \label{eq:train_feasible_cons}
    s.t. & \quad \xi(\hat{x}) \geq 0 \quad \forall \hat{x}\in \partial \mathcal{D}^{\gamma} \\
    \label{eq:train_correct_cons}
    & \quad \hat{b}_{\theta}(\hat{x}) \leq h(\hat{x}) \quad \forall \hat{x}\in \mathcal{X}\backslash\mathcal{D}^{\gamma}
\end{align}
where $\mathcal{D}^\gamma:=\{\hat{x}\mid \hat{b}^{\gamma}_{\theta}(\hat{x})\geq 0\}$. 
Here constraints \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} require parameter $\theta$ to define feasible and correct SNCBFs, respectively.
In what follows, we refer to \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} as feasibility and correct constraints.
Solving the constrained optimization problem is challenging. In this work, we convert the constrained optimization to an unconstrained one by constructing a loss function which penalizes violations of the constraints.
We then minimize the loss function over a training dataset to learn parameters $\theta$ and thus SNCBF $b_\theta$.
% A valid SNCBF is feasible as defined in Definition \ref{def:feasibility_scbf} and is correct defined in Definition \ref{def:correctness}. 
% Besides, a good SNCBF should not only be valid but also cover as much safe region as possible. We define an operator $Vol(\mathcal{D}_\gamma)$ represent the volume of the set $\mathcal{D}^{\gamma}$.  We next demonstrate how to synthesize a valid SNCBF. 
% To ensure the synthesized SCBF, we proposed the following loss function
% loss function design goes here

We denote the training dataset as $\mathcal{T}:=\{\hat{x}_{1}, \ldots, \hat{x}_{N}\mid \hat{x}_{i}
\in \mathcal{X}, \forall i =1,\ldots,N\}$, where $N$ is the number of samples. The dataset $\mathcal{T}$ is generated by simulating estimates with fixed point sampling in \cite{dawson2023safe}. We first uniformly discretize the state space into cells with length vector $L$. Next, we uniformly sample the center of discretized cell as fixed points $x_{f}$. Then we simulate the estimates by introducing a perturbation $\rho[j]$  sampled uniformly from interval $[x_{f}[j]-0.5 L[j], x_{f}[j]+0.5 L[j]]$. Finally, we have the sampling data $\hat{x}=x_{f}+\rho\in \mathcal{T}\subseteq \mathcal{X}$.
% The estimates $x_{R}$ are synthesized with $x_{f}$ perturbed by Gaussian noise, i.e., $x_{R}[j] = x_{f}[j] + \mathcal{N}(0, \sigma_{j}^2)$ where $\sigma_{j}$ is the standard deviation of corresponding sensor indexed $j$.

% Then a valid SNCBF can be trained using $\mathcal{T}$ by solving the following optimization program. 
% %The training of SNCBF can be summarized as a constrained optimization problem as follows. 
% \begin{align}
%     \label{eq:train_obj}
%     \max_{\theta}&\quad{Vol(\mathcal{D}^\gamma)} \\
%     \label{eq:train_feasible_cons}
%     s.t. & \quad \xi(\hat{x}) \geq 0 \quad \forall \hat{x}\in \partial \mathcal{D}^{\gamma} \\
%     \label{eq:train_correct_cons}
%     & \quad \hat{b}_{\theta}(\hat{x}) \leq h(\hat{x}) \quad \forall \hat{x}\in \mathcal{X}\backslash\mathcal{D}^{\gamma}
% \end{align}
% where $\mathcal{D}^\gamma:=\{\hat{x}\mid \hat{b}^{\gamma}_{\theta}(\hat{x})\geq 0\}$. 
% Here constraints \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} require parameter $\theta$ to define feasible and correct SNCBFs, respectively.
% In what follows, we refer to \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} as feasibility and correct constraints.
% Solving the constrained optimization problem is challenging. In this work, we convert the constrained optimization to an unconstrained one using the Lagrangian method \cite{hestenes1969multiplier}, which introduces a Lagrangian multiplier to penalize violations of the constraints. 
We then formulate the following unconstrained optimization problem to search for $\theta$
\begin{equation}
    \label{eq:uncons_opt}
    \min_{\theta}\quad{-Vol(\mathcal{D}_{\theta}^{\gamma})} + \lambda_{f}\mathcal{L}_f + \lambda_{c}\mathcal{L}_c 
\end{equation}
where $\mathcal{L}_f$ is the loss penalizing the violations of constraint \eqref{eq:train_feasible_cons}, $\mathcal{L}_c$ penalizes the violations of constraint \eqref{eq:train_correct_cons}, and $\lambda_{f}$ and $\lambda_{c}$ are nonnegative coefficients. 
The objective function \eqref{eq:train_obj} is approximated by the following quantity
\begin{equation}
    \label{eq:volume_obj}
    Vol(\mathcal{D}_{\theta}^{\gamma}) = \sum_{\hat{x}\in \mathcal{T}}{-ReLU(h(\hat{x}))ReLU(-b_{\theta}(\hat{x}))}. 
\end{equation}
The idea is to penalize samples $\hat{x}$ in the safety region but not in $\mathcal{D}^\gamma$, i.e., $h(\hat{x})>0$ and $b_\theta(\hat{x})<0$. 
The penalty of violating the feasibility constraint \eqref{eq:train_feasible_cons} is defined as
\begin{equation}\label{eq:Lf-SNCBF}
    \mathcal{L}_f = \sum_{\hat{x}\in \mathcal{T}} -\Delta(\hat{x}) ReLU(-\xi(\hat{x}) - \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u + \hat{b}(\hat{x})), 
\end{equation}
where $\Delta(\hat{x})$ is an indicator function such that $\Delta(\hat{x}):= 1$ if $b_{\theta}(\hat{x})=\overline{b}^{\gamma}$ and $\Delta(\hat{x}):= 0$ otherwise. The function $\Delta$ allows us to find and penalize sample points $\hat{x}$ satisfying $b_{\theta}(\hat{x})=0$ and  $\xi(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u <0 $.
% We penalize for the points that the following two condition hold
% \begin{enumerate}
%     \item $b_{\theta}(\hat{x})=0$.
%     \item $\xi(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u <0 $. 
% \end{enumerate}
For each sample $\hat{x}\in\mathcal{T}$, the control input $u$ in Eq. \eqref{eq:Lf-SNCBF} is computed as follows 
\begin{equation}
\begin{split}
    \min_{u} & \quad u^{T}u \\
    s.t. & \quad \xi(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u \geq 0
\end{split}
\end{equation}
The loss function to penalize the violations of the correctness constraint \eqref{eq:train_correct_cons} is constructed as 
\begin{equation}
    \label{eq:correctness_loss}
    \mathcal{L}_c = \sum_{\hat{x}\in \mathcal{T}}{ReLU(-h(\hat{x}))ReLU(b_{\theta}(\hat{x}))}
\end{equation}
The term $\mathcal{L}_c$ penalizes the samples $\hat{x}$ outside the safety region but being regarded safe, i.e., $h(\hat{x})<0$ and $b_{\theta}(\hat{x})>0$. 
When $\mathcal{L}_c$ and $\mathcal{L}_f$ converge to $0$, the feasibility and correctness constraints \eqref{eq:train_feasible_cons}- \eqref{eq:train_correct_cons} are satisfied.
% The proposed framework can either train a bank of SNCBF or a solo SNCBF that can further be used for safety constraint construction. 


\subsection{Synthesis of FT-SNCBF}
% Synthesis of FT-SNCBF 
% Fault-tolerent is an extension of SNCBF
% conclude what we have in previous section and introduce what we are going to have in this section
In the previous subsection, we described how to learn SNCBFs from data. In this subsection, we first generalize the feasibility and correctness properties for adversarial scenarios. 
We then construct a loss function to train a valid fault tolerant-SNCBF (FT-SNCBF) for all fault patterns.
% Specifically, we desire a function $b_{\theta}$ to satisfy the properties defined in Definition \ref{def:feasibility_scbf} and \ref{def:correctness}. 
% Based on the generalized properties, we next formulate a loss function to train a valid fault tolerant-SNCBF (FT-SNCBF) for all fault patterns.

Define \begin{equation*}
\overline{b}_{\theta}^{\gamma_{i}}
= \sup_{x,x^{0}}{\left\{b_{\theta}(\hat{x}) : ||x-x^{0}||_{2} \leq \gamma_{i}\right.} \\
\left. \text{ and } \hat{b}_{\theta}(x^{0})=0\right\}.
\end{equation*}
The following proposition gives the  necessary and sufficient conditions for a function $b_{\theta}$ to be an FT-SNCBF.  

\begin{proposition}
\label{prop:verify_ftscbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $b_{\theta}(\hat{x})$ is an FT-SNCBF if and only if there is no $\hat{x}\in \mathcal{D}^{\gamma_i}$, satisfying
$\frac{\partial b}{\partial x}g(\hat{x}) = 0$ , $\xi_{i}(\hat{x}) < 0$ for all $i\in Z_t$ where 
\begin{multline}
\label{eq:ftsncbf_cond}
    \xi_{i}(\hat{x}) =  \frac{\partial b}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x})K\nu\right) + \\
    ||\frac{\partial h}{\partial x}(\hat{x})K_{t,i}c||_{2} +  \hat{b}^{\gamma_i}(\hat{x}).
\end{multline}
and $\hat{b}_{\theta}^{\gamma_i}(\hat{x})=b_{\theta}(\hat{x})-\overline{b}^{\gamma}$
\end{proposition}
The proposition can be proved using the similar idea to Proposition \ref{prop:verify_scbf}. We omit the proof due to space constraint. 

We construct the following loss function to learn the FT-SNCBF 
\begin{equation}
    \label{eq:train_ftsncbf}
    \min_{\theta}\quad{-Vol(\mathcal{D}_{\theta}^{\gamma})} + \sum_{i\in Z_t}{\mathcal{L}^{i}_{f}} + \mathcal{L}_c. 
\end{equation}
% We define the objective function as \eqref{eq:volume_obj} and the correctness constraint as \eqref{eq:correctness_loss}. 
Note that a valid FT-SNCBF needs to satisfy the feasibility and correctness constraints.
The penalty of violating the feasibility constraint is defined as $\mathcal{L}_{f} = \sum_{i\in Z_t}{\mathcal{L}^{i}_{f}}$, where
\begin{equation*}
    \mathcal{L}^{i}_{f} = \sum_{\hat{x}\in \mathcal{T}} -\overline{\Delta}_{i}(\hat{x}) ReLU(-\xi_{i}(\hat{x}) - \frac{\partial b_{\theta}}{\partial x}(\hat{x}) u + \hat{b}^{\gamma_i}(\hat{x})), 
\end{equation*}
$\overline{\Delta}(\hat{x})$ is an indicate function such that $\overline{\Delta}(\hat{x}):= 1$ if $b_{\theta}(\hat{x})\leq\max_{i\in Z_t}{\{\overline{b}^{\gamma_i}\}}$ and $\Delta(\hat{x}):= 0$ otherwise. 
The control input $u$ used to compute $\mathcal{L}_f^i$ for each sample $\hat{x}$ is calculated as follows. 
\begin{equation}
\label{eq:ctrl_multiSNCBF}
\begin{split}
    \min_{u} & \quad u^{T}u \\
    s.t. & \quad \xi_{i}(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}(\hat{x}) u \geq 0 \quad \forall i\in Z_t
\end{split}
\end{equation}
When $\mathcal{L}_c$ and all $\mathcal{L}_f$ converge to $0$, the learned $b_{\theta}$ is a valid FT-SNCBF candidate. 
% Note that a good SNCBF candidate does not guarantee valid. The verification of a SNCBF candidate is needed and is a non-trivial process. 

\subsection{Fault Tolerant Framework}
% FT-Framework (Controller synthesis)
% EKF banks FT-framework
% Safety guarantee
% A training procedure is proposed in previous sections for SNCBF and FT-SNCBF. However, to ensure safety of a system, a fault-tolerant framework for safe control in non-trivial. Hence, we address this issue in this subsection. 

In this subsection, we present how to use the learned FT-SNCBF to synthesize a control input $u_t$ at each time $t$ such that the safety constraint is satisfied regardless of sensor faults and attacks.
We first employ an EKF to compute state estimates using all sensor measurements $\{1,\ldots,q\}$.
In addition, we maintain a set of EKFs to compute state estimates.
Each EKF is associated with the sensor measurements from $\{1,\ldots,q\}\setminus \mathcal{F}(r_i)$ for all $i=1,\ldots,m$, i.e., measurements obtained by excluding $\mathcal{F}(r_i)$.
We denote the state estimates obtained after excluding sensors associated with fault pattern $r_i$ as $\hat{x}_{t,i}$.



% In this subsection, we develop a fault tolerant framework which utilizes the learned FT-SNCBF to synthesize a control policy to guarantee safety.
We maintain $1+m+{m \choose 2}$ EKFs.
\begin{enumerate}
    \item $1$: One EKF is designed for fault free case. 
    \item $m$: Each EKF corresponds to a different possible fault pattern in $\{r_1,\dots r_m\}$. 
    \item ${m \choose 2}$: Each EKF corresponds to the combination of fault pattern $i,j\in\{r_1,\dots r_m\}$, $i\neq j$. 
\end{enumerate}
We ensure safety with probability $(1-\epsilon)$ by synthesizing a FT-SNCBF and construct $m+1$ corresponding constraints for each fault pattern on the control input. The deployment of the proposed FT-Framework can be summarized in the following Algorithm.
\begin{algorithm}[h]
\begin{algorithmic}[]
\caption{Fault-Tolerant Safe Control}
    \State \textbf{Input:} Sensor Input $y_{t}$, known fault pattern $\mathcal{F}$, trained FT-SNCBF $b_{\theta}$
    \State \textbf{Output:} Control Input $u$
    \Procedure{$u = FTC$}{$y_{t}\mid \mathcal{F}, b_{\theta}$}
    \State $\hat{x}_{t,0} \leftarrow EKF(y_{t,0})$.
    \For{$i,j \in \{1,\dots,m\}$ and $i\neq j$}
        \State $\hat{x}_{t,i} \leftarrow EKF(y_{t,i})$.
        \State $\hat{x}_{t,i,j} \leftarrow EKF(y_{t,i,j})$.
    \EndFor
    \State $Z_{t} \leftarrow \{1, \dots, m\}$. 
    \State Search for $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$ by solving \eqref{eq:ctrl_multiSNCBF}. 
    \Comment{Step 1}
    \If{No such $u_{t}$ can be found}
    \Comment{Step 2}
    \For{$i,j \in Z_t$ s.t. $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} > \theta_{ij}$} 
        \If{$||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} > \theta_{ij}/2$}
            \State $Z_{t} \leftarrow Z_{t} \setminus \{i\}$
        \Else
            \State $Z_{t} \leftarrow Z_{t} \setminus \{j\}$
        \EndIf
        \If{$\bigcap_{i \in Z_{t}}{\Omega_{i}} \neq \emptyset$}
            \State Search for $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$ by solving \eqref{eq:ctrl_multiSNCBF}. 
        \EndIf
    \EndFor
    \If{No such $u_{t}$ can be found}
        \Comment{Step 3}
        \State $i_{r} \leftarrow \min_{i}{\{\overline{y}_{t,i}-\overline{c}_{i}\hat{x}_{t,i}\}}$. 
        \State $Z_{t} \leftarrow \{i_{r}\}$.
        \State Search for $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$ by solving \eqref{eq:ctrl_multiSNCBF}. 
    \EndIf
    \EndIf
    \State \Return{$u_{t}$}
    \EndProcedure
\end{algorithmic}
\label{alg:ftcontrol}
\end{algorithm}

We next show the safety guarantee of the system under sensor faults. The following result gives sufficient conditions to guarantee safety. 
\begin{lemma}[\cite{clark2020control}]
    \label{lemma:ftsafe}
    Suppose  $\gamma_{1},\ldots,\gamma_{m}$, and $\theta_{ij}$ for $i < j$ are chosen such that the following conditions are satisfied:
    \begin{enumerate}
    \item Define  $\Lambda_{i}(\hat{x}_{t,i}) = \frac{\partial h_{i}}{\partial x}(\hat{x}_{t,i})g(\hat{x}_{t,i})$. There exists $\delta > 0$ such that for any $X_{t}^{\prime} \subseteq X_{t}(\delta)$ satisfying $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} \leq \theta_{ij}$ for all $i,j \in X_{t}^{\prime}$,  there exists $u$ such that
    \begin{equation}
    \label{eq:FT-CBF2}
    \Lambda_{i}(\hat{x}_{t,i})u > \xi_{i}(\hat{x})
    \end{equation}
    for all $i \in Z_{t}$.
    \item For each $i$, when $r=r_{i}$, 
    \begin{multline}
    \label{eq:FT-CBF3}
    Pr(||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \theta_{ij}/2 \ \forall j, ||\hat{x}_{t,i}-x_{t}||_{2} \leq \gamma_{i} \ \forall t)\\
     \geq 1-\epsilon.
    \end{multline}
    \end{enumerate}
    Then $Pr(x_{t} \in \mathcal{D} \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$.
\end{lemma}
However, Lemma \ref{lemma:ftsafe} depends on the existence of $u_{t}$. The following proposition provides sufficient condition of the existence of $u_{t}$ for all $\hat{x}\in \mathcal{D}^{\gamma_i}_{\theta}, \ \forall i\in Z_{t}$.  
\begin{proposition}
    \label{prop:u_f_ftsncbf}
    Suppose a FT-SNCBF $b_{\theta}$ satisfies the conditions in Proposition \ref{prop:verify_ftscbf} for $i\in Z_{t}$. Then, there always exists $u_{t}$ such that $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})u_{t}+\xi_{i}\geq 0$ $\forall \hat{x}\in \mathcal{D}_{\theta}^{\gamma_i}, \ \forall i\in Z_t$. 
\end{proposition}
\begin{proof}    
    We prove by showing there always exists $u_t$ such that \eqref{eq:SCBF-2} hold for two cases, namely, (i) $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})\neq0$ and (ii) $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})=0$. 
    For case (ii), we can always choose $u_{t}$ such that \eqref{eq:SCBF-2} holds for all $i\in Z_t$. For case (ii), there does not exist $\hat{x}$ such that $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})=0$ and $\xi_i(\hat{x})< 0$ by Proposition \ref{prop:verify_ftscbf}. Hence, $u_{t}$ can be any real value. 
\end{proof}
Finally, we present safety guarantee for system under sensor faults. 
\begin{theorem}[Safety Guarantee under Sensor Faults]
    \label{th:FT_Safety}
    Given a FT-SNCBF $b_{\theta}$ satisfies the conditions in Proposition \ref{prop:verify_ftscbf} for $i\in Z_{t}$. Suppose $\gamma_{1},\ldots,\gamma_{m}$, and $\theta_{ij}$ for $i < j$ are chosen such that conditions in \ref{lemma:ftsafe} hold. Then $Pr(x_{t} \in \mathcal{D} \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$. 
\end{theorem}
\begin{proof}
    By \cite[Theorem 3]{clark2020control} if there exist $u_{t}$ such that $\Omega_{i}$ holds 
    $\forall \hat{x}\in \mathcal{D}^{\gamma}_{\theta}$ $\forall i\in Z_{t}$ then, by Theorem \ref{theorem:SCBF}, 
    \begin{multline*}
    Pr(x_{t} \in \mathcal{D} \ \forall t | ||\hat{x}_{t,i}-\hat{x}_{t}||_{2} \leq \gamma_{i}, \\ ||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \theta_{ij}/2 \ \forall t) = 1
    \end{multline*}
    By Proposition \ref{prop:u_f_ftsncbf}, there exist $u_t$ s.t. $\Omega_{i}$ holds for all $\hat{x}\in \mathcal{D}^{\gamma_i}\quad \forall i\in Z_{t}$. 
    and $Pr(x_{t} \in \mathcal{D}\subseteq \mathcal{C} \ \forall t) > 1-\epsilon$ by (\ref{eq:FT-CBF3}).
\end{proof} 

% \subsection{FT-NCBF Design}
% The network is designed to take all estimates $\hat{x}_i$, $\forall i$ and indicator $I$. Intuitively, the indicator works like a mask to filter out unwanted estimates and activate different gain for corresponding $\gamma_i$

% \subsection{EKF Residual-based Fault Pattern Classification (Potential)}
% \textbf{Action needed **} The classification requires us to derive a guarantee. Fundamentally, the classifier is to make the whole design of the framework more cohesive by removing step 1, 2 and 3. 


==> sections/FTNCBF_v2.tex <==
% \section{Fault Tolerant NCBF}\label{sec:sol}
\section{Synthesis of Fault Tolerant SNCBF and Safety-Critical Control}\label{sec:sol}
% In this section we present the stochastic NCBFs (SNCBFs) and fault-tolerant SNCBFs (FT-SNCBFs). 
In this section, we first derive the necessary and sufficient conditions for SNCBFs. 
We further generalize SNCBFs and propose FT-SNCBFs.
We construct a loss function to learn FT-SNCBFs from data. 
We finally show how the learned FT-SNCBFs can be used for the synthesis of control inputs to guarantee safety.



% Background
% EKF
% SCBF
% FT-framework

% High level intuition
% (make sure that the details of overview will be coverd in the later subsections or can be found in other references)

% Synthesis of SNCBF (Training)
% theoretical foundation provide the criterion on what are good SNCBFs
% - correctness (how to check)
% - feasibility (derive condition for SNCBF feasibility)
% Training (Loss function design)
% Based on theroetical foundation, we design the loss function to guide SNCBF to converge

% Synthesis of FT-SNCBF 
% Fault-tolerent is an extension of SNCBF

% FT-Framework (Controller synthesis)
% EKF banks FT-framework
% Safety guarantee


% \subsection{Roadmap of Solution Methodology}

% We first derive the necessary and sufficient conditions for a function to be a stochastic neural control barrier function (SNCBF).
% We then construct a loss function using the derived conditions to learn SNCBF from data.
% While SNCBFs can be used for safety-critical control synthesis of robotic systems in benign environments, we generalize them and propose fault tolerant SNCBFs (FT-SNCBFs) for systems under sensor faults and attacks.
% We present a data-driven method to learn FT-SNCBFs.
% Given the learned FT-SNCBFs, we formulate a quadratic program for the synthesis of control inputs to satisfy the safety constraint.
% Specifically, we maintain a set of EKFs, with each being associated with one fault pattern.


% \subsection{Overview}
% % High level intuition
% % (make sure that the details of overview will be coverd in the later subsections or can be found in other references)
% Our goal is to synthesize a NCBF to play the role of SCBFs. To let one NCBF to replace the SCBFs corresponding to all possible fault patterns, we want to introduce the reasoning component as an input. The reasoning input belongs to a discrete space, indicating the fault patterns $I\in \mathcal{I}$, where $\mathcal{I}$ is the set of all possible fault patterns. To verify the FT-NCBF we verify $b_{\theta}(x\mid I)$, $\forall I\in \mathcal{I}$ where $I$ is the discrete input of fault patterns. In what follows, we will demonstrate our design of the pipeline. 


\subsection{Synthesis of SNCBF}\label{sec:SNCBF}
% Synthesis of SNCBF (Training)
% theoretical foundation provide the criterion on what are good SNCBFs
% - correctness (how to check)
% - feasibility (derive condition for SNCBF feasibility)
% Training (Loss function design)
% Based on theroetical foundation, we design the loss function to guide SNCBF to converge

% We generate with $b_{\theta}(x)$ with sensor noise and under different fault patterns. 

% Theorem to define a valid SCBF for polyCBF and NCBF
In this subsection, we describe how to synthesize SNCBFs. 
We first present the necessary and sufficient conditions for stochastic control barrier functions, among which SNCBFs constitute a special class represented by neural networks. 
% The safety of a stochastic system can be ensured safe by Theorem \ref{theorem:SCBF} given a function $b(x)$. In what follows, we shows criterion for SCBF candidates. 
% Let the estimation error to be represented as $z_t = (x_t-\hat{x}_t)$. 
% The following proposition gives the  necessary and sufficient conditions for a function $b$ to be a SCBF.  
\begin{proposition}
\label{prop:verify_scbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $b(\hat{x})$ is an SCBF if and only if there is no $\hat{x}\in \mathcal{D}^{\gamma}:=\{\hat{x}\mid \hat{b}(\hat{x})\geq 0\}$, satisfying
$\frac{\partial b}{\partial x}g(\hat{x}) = 0$ and $\xi^\gamma(\hat{x}) < 0$, where 
\begin{multline}
\label{eq:prop2cond}
    \xi^\gamma(\hat{x}) =  \frac{\partial b}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x})K\nu\right) + \\
    ||\frac{\partial b}{\partial x}(\hat{x})K_{t,i}c||_{2} +  \hat{b}^\gamma(\hat{x}).
\end{multline}
\end{proposition}
The proposition is derived based on \cite[Proposition 2]{zhang2022safe}. We omit the proof due to space constraint. 

We note that the class of SNCBFs is a special subset of SCBFs in Proposition \ref{prop:verify_scbf}. 
We denote the SNCBF as $b_\theta(\hat{x})$, where $\theta$ is the parameter of the neural network representing the function. 
We let  $\hat{b}_\theta^\gamma(\hat{x}) = b_\theta(\hat{x}) - \Bar{b}_\theta^\gamma$ and $\Bar{b}_\theta^\gamma = \sup_{\hat{x},\hat{x}^{0}}{\{b_\theta(\hat{x}) : ||\hat{x}-\hat{x}^{0}||_{2} \leq \gamma \text{ and } b_\theta(\hat{x}^{0})=0\}}.$
We further define
$\mathcal{D}_\theta=\{\hat{x}|b_\theta(\hat{x})\geq 0\}$ and 
$\mathcal{D}_\theta^\gamma=\{\hat{x}|\hat{b}_\theta^\gamma(\hat{x})\geq 0\}$.

In the following, we introduce the concept of \emph{valid} SNCBFs, and present how to synthesize them. 
A valid SNCBF needs to satisfy the following two properties.
\begin{definition}[Correct SNCBFs]
    \label{def:correctness}
    Given a safety region $\mathcal{C}$, the SNCBF $b_{\theta}$ is correct if and only if $\mathcal{D}_{\theta}\subseteq \mathcal{C}$. 
\end{definition}
The correctness property in Definition \ref{def:correctness} can be leveraged to ensure the positive invariance of set $\mathcal{D}_\theta$, and thus $\mathcal{C}$.
\begin{definition}[Feasible SNCBF]
\label{def:feasibility_scbf}
    The SNCBF $b_\theta$ parameterized by $\theta$ is feasible if and only if $\forall \hat{x}\in \mathcal{D}_\theta^{\gamma}$, $\exists u$ s.t. $\xi_\theta^\gamma(\hat{x}) + \frac{\partial b_\theta}{\partial x}g(\hat{x})u\geq 0$, where
    \begin{multline} \label{eq:prop2cond}
    \xi_\theta^\gamma(\hat{x}) =  \frac{\partial b_\theta}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}b_\theta}{\partial x^{2}}(\hat{x})K\nu\right) + \\
    ||\frac{\partial b_\theta}{\partial x}(\hat{x})K_{t,i}c||_{2} +  \hat{b}_\theta^\gamma(\hat{x}).
\end{multline}
\end{definition}
The feasibility property in Definition \ref{def:feasibility_scbf} ensures that a control input $u$ can always be found to satisfy inequality \eqref{eq:SCBF-2}, and hence can guarantee safety.
% Based on Proposition \ref{prop:verify_scbf} and Definition \ref{def:feasibility}, feasible SNCBFs can be defined as follows. 

% \begin{definition}[Feasible SNCBF]
% \label{def:feasibility_scbf}
%     The SNCBF $b_\theta$ parameterized by $\theta$ is feasible if and only if $\forall \hat{x}\in \mathcal{D}^{\gamma}$, $\exists u$ s.t. $\xi(\hat{x}) + \frac{\partial b_\theta}{\partial x}g(\hat{x})u\geq 0$. 
% \end{definition}

% Besides the feasibility property given in Definition \ref{def:feasibility_scbf}, a valid SNCBF $b_\theta$ also needs to be correct as shown in Definition \ref{def:correctness}. 
We note that there may exist infinitely many valid SNCBFs, making the synthesis of valid SNCBFs computationally expensive. In this work, we focus on synthesizing valid SNCBFs that encompass the largest possible safety region. To this end, we define an operator $Vol(\mathcal{D}_\theta)$ to represent the volume of the set $\mathcal{D}_\theta$, and synthesize a valid SNCBF such that $Vol(\mathcal{D}_\theta)$ is maximized. The optimization program is given as follows
\begin{align}
    \label{eq:train_obj}
    \max_{\theta}&\quad{Vol(\mathcal{D}_\theta)} \\
    \label{eq:train_feasible_cons}
    s.t. & \quad \xi_\theta^\gamma(\hat{x}) \geq 0 \quad \forall \hat{x}\in \partial \mathcal{D}_\theta^{\gamma} \\
    \label{eq:train_correct_cons}
    & \quad b_{\theta}(\hat{x}) \leq h(\hat{x}) \quad \forall \hat{x}\in \mathcal{X}\backslash\mathcal{D}_\theta
\end{align}
% where $\mathcal{D}^\gamma:=\{\hat{x}\mid \hat{b}^{\gamma}_{\theta}(\hat{x})\geq 0\}$. 
Here constraints \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} require parameter $\theta$ to define feasible and correct SNCBFs, respectively.
In what follows, we refer to \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} as feasibility and correctness constraints.
Solving the constrained optimization problem is challenging. In this work, we convert the constrained optimization to an unconstrained one by constructing a loss function which penalizes violations of the constraints.
We then minimize the loss function over a training dataset to learn parameters $\theta$ and thus SNCBF $b_\theta$.
% A valid SNCBF is feasible as defined in Definition \ref{def:feasibility_scbf} and is correct defined in Definition \ref{def:correctness}. 
% Besides, a good SNCBF should not only be valid but also cover as much safe region as possible. We define an operator $Vol(\mathcal{D}_\gamma)$ represent the volume of the set $\mathcal{D}^{\gamma}$.  We next demonstrate how to synthesize a valid SNCBF. 
% To ensure the synthesized SCBF, we proposed the following loss function
% loss function design goes here

We denote the training dataset as $\mathcal{T}:=\{\hat{x}_{1}, \ldots, \hat{x}_{N}\mid \hat{x}_{i}
\in \mathcal{X}, \forall i =1,\ldots,N\}$, where $N$ is the number of samples. The dataset $\mathcal{T}$ is generated by simulating estimates with fixed point sampling in \cite{dawson2023safe}. We first uniformly discretize the state space into cells with length vector $L$. Next, we uniformly sample the center of discretized cell as fixed points $x_{f}$. Then we simulate the estimates by introducing a perturbation $\rho[j]$  sampled uniformly from interval $[x_{f}[j]-0.5 L[j], x_{f}[j]+0.5 L[j]]$. Finally, we have the sampling data $\hat{x}_i=x_{f}+\rho\in \mathcal{T}\subseteq \mathcal{X}$.
% The estimates $x_{R}$ are synthesized with $x_{f}$ perturbed by Gaussian noise, i.e., $x_{R}[j] = x_{f}[j] + \mathcal{N}(0, \sigma_{j}^2)$ where $\sigma_{j}$ is the standard deviation of corresponding sensor indexed $j$.

% Then a valid SNCBF can be trained using $\mathcal{T}$ by solving the following optimization program. 
% %The training of SNCBF can be summarized as a constrained optimization problem as follows. 
% \begin{align}
%     \label{eq:train_obj}
%     \max_{\theta}&\quad{Vol(\mathcal{D}^\gamma)} \\
%     \label{eq:train_feasible_cons}
%     s.t. & \quad \xi(\hat{x}) \geq 0 \quad \forall \hat{x}\in \partial \mathcal{D}^{\gamma} \\
%     \label{eq:train_correct_cons}
%     & \quad \hat{b}_{\theta}(\hat{x}) \leq h(\hat{x}) \quad \forall \hat{x}\in \mathcal{X}\backslash\mathcal{D}^{\gamma}
% \end{align}
% where $\mathcal{D}^\gamma:=\{\hat{x}\mid \hat{b}^{\gamma}_{\theta}(\hat{x})\geq 0\}$. 
% Here constraints \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} require parameter $\theta$ to define feasible and correct SNCBFs, respectively.
% In what follows, we refer to \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} as feasibility and correct constraints.
% Solving the constrained optimization problem is challenging. In this work, we convert the constrained optimization to an unconstrained one using the Lagrangian method \cite{hestenes1969multiplier}, which introduces a Lagrangian multiplier to penalize violations of the constraints. 
We then formulate the following unconstrained optimization problem to search for $\theta$
\begin{equation}
    \label{eq:uncons_opt}
    \min_{\theta}\quad{-Vol(\mathcal{D}_{\theta})} + \lambda_{f}\mathcal{L}_f + \lambda_{c}\mathcal{L}_c 
\end{equation}
where $\mathcal{L}_f$ is the loss penalizing the violations of constraint \eqref{eq:train_feasible_cons}, $\mathcal{L}_c$ penalizes the violations of constraint \eqref{eq:train_correct_cons}, and $\lambda_{f}$ and $\lambda_{c}$ are nonnegative coefficients. 
The objective function \eqref{eq:train_obj} is approximated by the following quantity
\begin{equation}
    \label{eq:volume_obj}
    Vol(\mathcal{D}_{\theta}) = \sum_{\hat{x}\in \mathcal{T}}{-ReLU(h(\hat{x}))ReLU(-b_{\theta}(\hat{x}))}. 
\end{equation}
The idea is to penalize samples $\hat{x}$ in the safety region but not in $\mathcal{D}^\gamma$, i.e., $h(\hat{x})>0$ and $b_\theta(\hat{x})<0$. 
The penalty of violating the feasibility constraint \eqref{eq:train_feasible_cons} is defined as
\begin{equation}\label{eq:Lf-SNCBF}
    \mathcal{L}_f = \sum_{\hat{x}\in \mathcal{T}} -\Delta(\hat{x}) ReLU(-\xi_\theta^\gamma(\hat{x}) - \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u + \hat{b}^\gamma_\theta(\hat{x})), 
\end{equation}
where $\Delta(\hat{x})$ is an indicator function such that $\Delta(\hat{x}):= 1$ if $b_{\theta}(\hat{x})=\overline{b}^{\gamma}_\theta$ and $\Delta(\hat{x}):= 0$ otherwise. The function $\Delta$ allows us to find and penalize sample points $\hat{x}$ satisfying $\hat{b}_{\theta}^\gamma(\hat{x})=0$ and  $\xi_\theta^\gamma(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u <0 $.
% We penalize for the points that the following two condition hold
% \begin{enumerate}
%     \item $b_{\theta}(\hat{x})=0$.
%     \item $\xi(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u <0 $. 
% \end{enumerate}
For each sample $\hat{x}\in\mathcal{T}$, the control input $u$ in Eq. \eqref{eq:Lf-SNCBF} is computed as follows 
\begin{equation}
\begin{split}
    \min_{u} & \quad u^{T}u \\
    s.t. & \quad \xi_\theta^\gamma(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u \geq 0
\end{split}
\end{equation}
The loss function to penalize the violations of the correctness constraint \eqref{eq:train_correct_cons} is constructed as 
\begin{equation}
    \label{eq:correctness_loss}
    \mathcal{L}_c = \sum_{\hat{x}\in \mathcal{T}}{ReLU(-h(\hat{x}))ReLU(b_{\theta}(\hat{x}))}
\end{equation}
The term $\mathcal{L}_c$ penalizes the samples $\hat{x}$ outside the safety region but being regarded safe, i.e., $h(\hat{x})<0$ and $b_{\theta}(\hat{x})>0$. 
When $\mathcal{L}_c$ and $\mathcal{L}_f$ converge to $0$, the feasibility and correctness constraints \eqref{eq:train_feasible_cons}-\eqref{eq:train_correct_cons} are satisfied.
% The proposed framework can either train a bank of SNCBF or a solo SNCBF that can further be used for safety constraint construction. 


\subsection{Synthesis of FT-SNCBF}
% Synthesis of FT-SNCBF 
% Fault-tolerent is an extension of SNCBF
% conclude what we have in previous section and introduce what we are going to have in this section
% In the previous subsection, we described how to learn SNCBFs from data. 
In this subsection, we generalize the SNCBFs and propose fault tolerant SNCBFs (FT-SNCBFs) for system \eqref{eq:state-sde}-\eqref{eq:output-sde} under sensor faults and attacks.
We construct a loss function to train a valid FT-SNCBF for all fault patterns.
With a slight abuse of notations, we use $b_\theta$ to denote the FT-SNCBF in the remainder of this paper. 
% Notations $\hat{b}_\theta^\gamma(\hat{x})$, $\Bar{b}_\theta^\gamma$, $\mathcal{D}_\theta$, and  $\mathcal{D}_\theta^\gamma$ are defined in a similar fashion as we did in Section \ref{sec:SNCBF}.
% Specifically, we desire a function $b_{\theta}$ to satisfy the properties defined in Definition \ref{def:feasibility_scbf} and \ref{def:correctness}. 
% Based on the generalized properties, we next formulate a loss function to train a valid fault tolerant-SNCBF (FT-SNCBF) for all fault patterns.
We define $\hat{b}_\theta^{\gamma_i}(\hat{x})=b_\theta(\hat{x})-\Bar{b}_\theta^{\gamma_i}(\hat{x})$, where
\begin{equation*}
\overline{b}_{\theta}^{\gamma_{i}}
= \sup_{\hat{x},\hat{x}^{0}}{\left\{b_{\theta}(\hat{x}) : ||\hat{x}-\hat{x}^{0}||_{2} \leq \gamma_{i}\right.} \\
\left. \text{ and } b_{\theta}(\hat{x}^{0})=0\right\}.
\end{equation*}
%We further let $\mathcal{D}_\theta^{\gamma_i}=\{\hat{x}\mid \hat{b}_\theta^{\gamma_i}(\hat{x})\geq 0\}$.
The following proposition gives the  necessary and sufficient conditions for a function $b_{\theta}$ to be an FT-SNCBF.  

\begin{proposition}
\label{prop:verify_ftscbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $b_{\theta}(\hat{x})$ is an FT-SNCBF if and only if there is no $\hat{x}\in \mathcal{D}_\theta^{\gamma_i}$, satisfying
$\frac{\partial b_\theta}{\partial x}g(\hat{x}) = 0$ , $\xi_\theta^{\gamma_i}(\hat{x}) < 0$ for all $i\in \{1,\ldots,m\}$ where 
\begin{multline}
\label{eq:ftsncbf_cond}
    \xi_\theta^{\gamma_i}(\hat{x}) =  \frac{\partial b_\theta}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}b_\theta}{\partial x^{2}}(\hat{x})K\nu\right) + \\
    ||\frac{\partial h}{\partial x}(\hat{x})K_{t,i}c||_{2} +  \hat{b}^{\gamma_i}_\theta(\hat{x}).
\end{multline}
\end{proposition}
The proposition can be proved using the similar idea to Proposition \ref{prop:verify_scbf}. We omit the proof due to space constraint. 

We construct the following loss function to learn the FT-SNCBF 
\begin{equation}
    \label{eq:train_ftsncbf}
    \min_{\theta}\quad{-Vol(\mathcal{D}_{\theta})} + \lambda_f\sum_{i\in \{1,\ldots,m\}}{\mathcal{L}^{i}_{f}} + \lambda_c\mathcal{L}_c, 
\end{equation}
% We define the objective function as \eqref{eq:volume_obj} and the correctness constraint as \eqref{eq:correctness_loss}. 
where $\mathcal{L}_{f} = \sum_{i\in \{1,\ldots,m\}}{\mathcal{L}^{i}_{f}}$ is the penalty of violating the feasibility constraint,
\begin{equation*}
    \mathcal{L}^{i}_{f} = \sum_{\hat{x}\in \mathcal{T}} -\overline{\Delta}_{i}(\hat{x}) ReLU(-\xi_\theta^{\gamma_i}(\hat{x}) - \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u + \hat{b}_\theta^{\gamma_i}(\hat{x})), 
\end{equation*}
and $\overline{\Delta}(\hat{x})$ is an indicator function such that $\overline{\Delta}(\hat{x}):= 1$ if $b_{\theta}(\hat{x})\leq\max_{i\in Z_t}{\{\overline{b}^{\gamma_i}_\theta\}}$ and $\overline{\Delta}(\hat{x}):= 0$ otherwise. 
The control input $u$ used to compute $\mathcal{L}_f^i$ for each sample $\hat{x}$ is calculated as follows. 
\begin{equation}
\label{eq:ctrl_multiSNCBF}
\begin{split}
    \min_{u} & \quad u^{T}u \\
    s.t. & \quad \xi_\theta^{\gamma_i}(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u \geq 0 \quad \forall i\in Z_t
\end{split}
\end{equation}
When $\mathcal{L}_c$ and $\mathcal{L}_f$ converge to $0$, the learned $b_{\theta}$ is a valid FT-SNCBF. 
% Note that a good SNCBF candidate does not guarantee valid. The verification of a SNCBF candidate is needed and is a non-trivial process. 

\subsection{Safety-Critical Control Synthesis using FT-SNCBF}
% FT-Framework (Controller synthesis)
% EKF banks FT-framework
% Safety guarantee
% A training procedure is proposed in previous sections for SNCBF and FT-SNCBF. However, to ensure safety of a system, a fault-tolerant framework for safe control in non-trivial. Hence, we address this issue in this subsection. 

In this subsection, we present how to use the learned FT-SNCBF to synthesize a control input $u_t$ at each time $t$ such that the safety constraint is satisfied regardless of sensor faults and attacks.
% We first employ an EKF to compute state estimates using all sensor measurements $\{1,\ldots,q\}$.
We maintain a set of EKFs to compute state estimates.
Each EKF is associated with the sensor measurements from $\{1,\ldots,q\}\setminus \mathcal{F}(r_i)$ for all $i=1,\ldots,m$, i.e., measurements obtained by excluding $\mathcal{F}(r_i)$.
We denote the state estimates obtained after excluding sensors associated with fault pattern $r_i$ as $\hat{x}_{t,i}$.
We define 
\begin{equation*}
    \Omega_i = \{u:\xi_\theta^{\gamma_i} + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u \geq 0\}
\end{equation*}
as the feasible region when searching for control input under fault pattern $r_i$
Then if there exists a control input $u\in\cap_{i=1}^m\Omega_i\neq\emptyset$, such a control input can guarantee the safety under any fault pattern $r_i$.

It may not be viable to guarantee the existence of a control input $u$ satisfying constraints specified by $\Omega_i,\ldots,\Omega_m$ simultaneously due to sensor faults and attacks.
Thus we develop a mechanism to identify constraints conflicting with each other, and resolve such conflicts.
Our idea is to additionally maintain ${m \choose 2}$ EKFs, where each EKF computes state estimates using sensors from $\{1,\ldots,q\}\setminus(\mathcal{F}(r_i)\cup\mathcal{F}(r_j))$ for all $i\neq j$.
We use a variable $Z_t$ to keep track of the fault patterns that will not raise conflicts.
The variable $Z_t$ is initialized as $\{1,\ldots,m\}$.
If $\cap_{i\in Z_t}\Omega_i=\emptyset$, we compare state estimates $\hat{x}_{t,i}$ with $\hat{x}_{t,j}$ for all $i,j\in Z_t$ and $i\neq j$.
If $\|\hat{x}_{t,i}-\hat{x}_{t,i}\|_2\geq \alpha_{ij}$ for some chosen parameter $\alpha_{ij}>0$, then $Z_t$ is updated as 
\begin{equation*}
    Z_t = \begin{cases}
        Z_t\setminus \{i\},&\mbox{ if }\|\hat{x}_{t,i}-\hat{x}_{t,i,j}\|_2\geq \alpha_{ij}/2\\
        Z_t\setminus \{j\},&\mbox{ if }\|\hat{x}_{t,j}-\hat{x}_{t,i,j}\|_2\geq \alpha_{ij}/2
    \end{cases}.
\end{equation*}
After updating $Z_t$, if $\cap_{i\in Z_t}\Omega_i\neq\emptyset$, then control input $u_t$ can be chosen as
\begin{equation}\label{eq:control synthesis}
    \min_{u_t\in\cap_{i\in Z_t}\Omega_i}~u_t^Tu_t.
\end{equation}
Otherwise, we will remove indices $i$ corresponding to fault pattern $r_i$ that leads to largest residue $\Bar{y}_{t,i}-\Bar{c}_i\hat{x}_{t,i}$ until $\cap_{i\in Z_t}\Omega_i\neq \emptyset$.
Here $\Bar{y}_{t,i}$ is the output from sensors in $\{1,\ldots,q\}\setminus \mathcal{F}(r_i)$.

We summarize the procedure for synthesizing control inputs using FT-SNCBF in Algorithm \ref{alg:ftcontrol}. 
In what follows, we present the safety guarantee of our approach.

% In this subsection, we develop a fault tolerant framework which utilizes the learned FT-SNCBF to synthesize a control policy to guarantee safety.
% We maintain $1+m+{m \choose 2}$ EKFs.
% \begin{enumerate}
%     \item $1$: One EKF is designed for fault free case. 
%     \item $m$: Each EKF corresponds to a different possible fault pattern in $\{r_1,\dots r_m\}$. 
%     \item ${m \choose 2}$: Each EKF corresponds to the combination of fault pattern $i,j\in\{r_1,\dots r_m\}$, $i\neq j$. 
% \end{enumerate}
% We ensure safety with probability $(1-\epsilon)$ by synthesizing a FT-SNCBF and construct $m+1$ corresponding constraints for each fault pattern on the control input. The deployment of the proposed FT-Framework can be summarized in the following Algorithm.
\begin{algorithm}[h]
\begin{algorithmic}[]
\caption{Safety-Critical Control Synthesis using FT-SNCBF}\label{alg:ftcontrol}
    \State \textbf{Input:} Sensor measurements $y_{t}$, collection of fault patterns $r_1,\ldots,r_m$, learned FT-SNCBF $b_{\theta}$
    \State \textbf{Output:} Control Input $u_t$
    % \Procedure{$u = FTC$}{$y_{t}\mid \mathcal{F}, b_{\theta}$}
    % \State $\hat{x}_{t} \leftarrow EKF(y_{t})$
        \State $\hat{x}_{t,i} \leftarrow EKF(\Bar{y}_{t,i})$ for all $i\in \{1,\dots,m\}$
        \State $\hat{x}_{t,i,j} \leftarrow EKF(\Bar{y}_{t,i,j})$ for all $i,j \in \{1,\dots,m\}$ and $i\neq j$
    \State $Z_{t} \leftarrow \{1, \dots, m\}$
    \While {$\cap_{i\in Z_t}\Omega_i=\emptyset$}
    \For{$i,j \in Z_t$ such that $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} > \alpha_{ij}$} 
        \If{$||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} > \alpha_{ij}/2$}
            \State $Z_{t} \leftarrow Z_{t} \setminus \{i\}$
        \ElsIf{$||\hat{x}_{t,j}-\hat{x}_{t,i,j}||_{2} > \alpha_{ij}/2$}
            \State $Z_{t} \leftarrow Z_{t} \setminus \{j\}$
        \EndIf
    \EndFor
    \If{$\bigcap_{i \in Z_{t}}{\Omega_{i}} \neq \emptyset$}
            \State Compute $u_t$ using Eq. \eqref{eq:control synthesis}
            \State \textbf{Return $u_t$}
    \Else
    \State $i_{r} \leftarrow \arg\max_{i}{\{\overline{y}_{t,i}-\overline{c}_{i}\hat{x}_{t,i}\}}$. 
    \State $Z_{t} \leftarrow Z_t\setminus\{i_{r}\}$.
    \EndIf
    \EndWhile
    % \EndProcedure
\end{algorithmic}
\end{algorithm}

We next show the safety guarantee of the system under sensor faults. The following result gives the sufficient conditions of safety. 
\begin{lemma}[\cite{clark2020control}]
    \label{lemma:ftsafe}
    Suppose  $\gamma_{1},\ldots,\gamma_{m}$, and $\alpha_{ij}$ for $i < j$ are chosen such that the following conditions are satisfied:
    \begin{enumerate}
    \item Define  $\Lambda_{i}(\hat{x}_{t,i}) = \frac{\partial b_\theta^{\gamma_i}}{\partial x}g(\hat{x}_{t,i})$. There exists $\delta > 0$ such that for any $X_{t}^{\prime} \subseteq X_{t}(\delta):=\{i\mid \hat{b}_{\theta}^{\gamma_i}(\hat{x}_{t,i})<\delta\}$ satisfying $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} \leq \alpha_{ij}$ for all $i,j \in X_{t}^{\prime}$,  there exists $u$ such that
    \begin{equation}
    \label{eq:FT-CBF2}
    \Lambda_{i}(\hat{x}_{t,i})u > -\xi_\theta^{\gamma_i}
    \end{equation}
    for all $i \in Z_t$.
    \item For each $i$, when $r=r_{i}$, 
    \begin{multline}
    \label{eq:FT-CBF3}
    Pr(||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \alpha_{ij}/2 \ \forall j, ||\hat{x}_{t,i}-x_{t}||_{2} \leq \gamma_{i} \ \forall t)\\
     \geq 1-\epsilon.
    \end{multline}
    \end{enumerate}
    Then $Pr(x_{t} \in \mathcal{D}_\theta \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$.
\end{lemma}
However, Lemma \ref{lemma:ftsafe} depends on the existence of $u_{t}$. The following proposition provides sufficient condition of the existence of $u_{t}$ for all $\hat{x}\in \mathcal{D}^{\gamma_i}_{\theta}, \ \forall i\in Z_{t}$.  
\begin{proposition}
    \label{prop:u_f_ftsncbf}
    Suppose an FT-SNCBF $b_{\theta}$ makes losses $\mathcal{L}_f+\mathcal{L}_c\rightarrow 0$ as the training dataset $\mathcal{T}$ approaches $\mathcal{X}$.
    Then, there always exists $u_{t}$ such that $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})u_{t}+\xi_\theta^{\gamma_i}\geq 0$ $\forall \hat{x}\in \mathcal{D}_{\theta}^{\gamma_i}, \ \forall i\in Z_t$. 
\end{proposition}
\begin{proof}
    By the constructions of $\mathcal{L}_f^i$ and $\mathcal{L}_c$, we first note that these losses are non-negative. Thus if $\mathcal{L}_f+\mathcal{L}_c\rightarrow 0$, we must have that $\mathcal{L}_f^i,\mathcal{L}_f,\mathcal{L}_c\rightarrow 0$.
    According to the definitions of $\mathcal{L}_f$ and $\mathcal{L}_f^i$, we then have that there must exist some control input $u$ that solves the optimization program in Eq. \eqref{eq:ctrl_multiSNCBF} when  $\mathcal{L}_f^i,\mathcal{L}_f\rightarrow 0$. Otherwise losses $\mathcal{L}_f^i$ and $\mathcal{L}_f$ will be positive.
\end{proof}
% \begin{proposition}
%     \label{prop:u_f_ftsncbf}
%     Suppose a FT-SNCBF $b_{\theta}$ satisfies the conditions in Proposition \ref{prop:verify_ftscbf} for $i\in Z_{t}$. Then, there always exists $u_{t}$ such that $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})u_{t}+\xi_{i}\geq 0$ $\forall \hat{x}\in \mathcal{D}_{\theta}^{\gamma_i}, \ \forall i\in Z_t$. 
% \end{proposition}
% \begin{proof}    
%     We prove by showing there always exists $u_t$ such that \eqref{eq:SCBF-2} hold for two cases, namely, (i) $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})\neq0$ and (ii) $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})=0$. 
%     For case (ii), we can always choose $u_{t}$ such that \eqref{eq:SCBF-2} holds for all $i\in Z_t$. For case (ii), there does not exist $\hat{x}$ such that $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})=0$ and $\xi_i(\hat{x})< 0$ by Proposition \ref{prop:verify_ftscbf}. Hence, $u_{t}$ can be any real value. 
% \end{proof}
We finally conclude this section by presenting the safety guarantee provided by our approach. 
\begin{theorem}[Safety Guarantee under Sensor Faults]
    \label{th:FT_Safety}
    Let $b_{\theta}$ be an FT-SNCBF such that $\mathcal{L}_f+\mathcal{L}_c\rightarrow 0$ as the training dataset $\mathcal{T}$ approaches $\mathcal{X}$. 
    Suppose $\gamma_{1},\ldots,\gamma_{m}$, and $\alpha_{ij}$ for $i < j$ are chosen such that the conditions in Lemma \ref{lemma:ftsafe} hold. Then $Pr(x_{t} \in \mathcal{D} \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$. 
\end{theorem}
\begin{proof}
    The theorem immediately follows from Lemma \ref{lemma:ftsafe} and Proposition \ref{prop:verify_ftscbf}.
\end{proof}
% \begin{theorem}[Safety Guarantee under Sensor Faults]
%     \label{th:FT_Safety}
%     Given an FT-SNCBF $b_{\theta}$ satisfies the conditions in Proposition \ref{prop:verify_ftscbf} for $i\in Z_{t}$. Suppose $\gamma_{1},\ldots,\gamma_{m}$, and $\theta_{ij}$ for $i < j$ are chosen such that conditions in \ref{lemma:ftsafe} hold. Then $Pr(x_{t} \in \mathcal{D} \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$. 
% \end{theorem}
% \begin{proof}
%     By \cite[Theorem 3]{clark2020control} if there exist $u_{t}$ such that $\Omega_{i}$ holds 
%     $\forall \hat{x}\in \mathcal{D}^{\gamma}_{\theta}$ $\forall i\in Z_{t}$ then, by Theorem \ref{theorem:SCBF}, 
%     \begin{multline*}
%     Pr(x_{t} \in \mathcal{D} \ \forall t | ||\hat{x}_{t,i}-\hat{x}_{t}||_{2} \leq \gamma_{i}, \\ ||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \theta_{ij}/2 \ \forall t) = 1
%     \end{multline*}
%     By Proposition \ref{prop:u_f_ftsncbf}, there exist $u_t$ s.t. $\Omega_{i}$ holds for all $\hat{x}\in \mathcal{D}^{\gamma_i}\quad \forall i\in Z_{t}$. 
%     and $Pr(x_{t} \in \mathcal{D}\subseteq \mathcal{C} \ \forall t) > 1-\epsilon$ by (\ref{eq:FT-CBF3}).
% \end{proof} 

% \subsection{FT-NCBF Design}
% The network is designed to take all estimates $\hat{x}_i$, $\forall i$ and indicator $I$. Intuitively, the indicator works like a mask to filter out unwanted estimates and activate different gain for corresponding $\gamma_i$

% \subsection{EKF Residual-based Fault Pattern Classification (Potential)}
% \textbf{Action needed **} The classification requires us to derive a guarantee. Fundamentally, the classifier is to make the whole design of the framework more cohesive by removing step 1, 2 and 3. 


==> sections/FTNCBF_v3.tex <==
% \section{Fault Tolerant NCBF}\label{sec:sol}
\section{Solution Approach to Safety-Critical Control and Synthesis of Fault Tolerant NCBF}\label{sec:sol}
% In this section we present the stochastic NCBFs (SNCBFs) and fault-tolerant SNCBFs (FT-SNCBFs). 

In this section, we first present an overview on how to synthesize control inputs for the system in \eqref{eq:state-sde}-\eqref{eq:output-sde} such that safety can be guaranteed under sensor faults and attacks.
The key to our approach is the development of a new class of control barrier functions named fault tolerant neural control barrier functions (FT-NCBFs).
We derive the necessary and sufficient conditions for FT-NCBFs, and construct a loss function to learn FT-NCBFs from data.

\subsection{Overview of the Proposed Solution Approach}

This subsection presents an overview of our proposed solution approach to safety-critical control synthesis.
The solution is inspired by the CBF-based approaches.
Our insight is that when the attack pattern is unknown, safety can be guaranteed if we can synthesize an NCBF for the robot in \eqref{eq:state-sde}-\eqref{eq:output-sde} such that the there exists a control input that steers the robot towards the interior of the positive invariant set corresponding to the NCBF under all potential faults and attacks.
We term this NCBF as fault tolerant neural control barrier function (FT-NCBF) and define it as follows.
\begin{definition}
    A function $b_\theta$ parameterized by $\theta$ is said to be a fault tolerant neural control barrier function for the system in \eqref{eq:state-sde}-\eqref{eq:output-sde} if there exists a control input $u$ such that under all attack patterns $r_i\in\{r_1,\ldots,r_m\}$,
    \begin{multline}
        \frac{\partial b_\theta}{\partial x}f(\hat{x}_{t,i}) +  \frac{\partial b_\theta}{\partial x}g(\hat{x}_{t,i})u + \frac{1}{2}\mathbf{tr}\left(\nu^{T}K_{t,i}^{T}\frac{\partial^{2}b_\theta}{\partial x^{2}}(\hat{x}_{t,i})K_{t,i}\nu\right)  \\
    -\gamma\|\frac{\partial b_\theta}{\partial x}(\hat{x}_{t,i})K_{t,i}c\|_{2} +  \hat{b}^{\gamma_i}_\theta(\hat{x}_{t,i})\geq 0
    \end{multline}
    for all $\hat{x}_{t,i}$ satisfying $b_\theta^\gamma(\hat{x}_{t,i}):=b_\theta(\hat{x}_{t,i})-\Bar{b}_\theta^\gamma\geq 0$ and $\|\hat{x}_{t,i}-x_t\|\leq \gamma$, where $\hat{x}_{t,i}$ is the state estimate by Eq. \eqref{eq:ekf} using outputs from $\{1,\ldots,q\}\setminus \mathcal{F}(r_i)$, and $$\Bar{b}_\theta^\gamma = \sup_{\hat{x},\hat{x}^{0}}{\{b_\theta(\hat{x}) : ||\hat{x}-\hat{x}^{0}||_{2} \leq \gamma \text{ and } b_\theta(\hat{x}^{0})=0\}}.$$
\end{definition}

The key to our solution approach is the synthesis of FT-NCBFs. 
In the remainder of this section, we first investigate how to synthesize NCBFs for the robot in Eq. \eqref{eq:state-sde}-\eqref{eq:output-sde} when there exists no adversary (Section \ref{sec:SNCBF}).
We then use the NCBFs as a building block, and present how to synthesize FT-NCBFs.
We construct a loss function to learn FT-NCBFs in Section \ref{sec:FT-NCBF}.
We finally discuss how the proposed FT-NCBFs can be utilized for control synthesis and the safety guarantee (Section \ref{sec:conflict}).

% In the remainder of this section, we formalize this insight by first deriving the necessary and sufficient conditions for NCBFS of robots modeled by Eq. \eqref{eq:state-sde}-\eqref{eq:output-sde} in the absence of adversary (Section \ref{sec:SNCBF}).
% We then generalize the conditions for NCBFs and synthesize FT-NCBFs for robots under sensor faults and attacks. 







\subsection{Synthesis of NCBF}\label{sec:SNCBF}
% Synthesis of SNCBF (Training)
% theoretical foundation provide the criterion on what are good SNCBFs
% - correctness (how to check)
% - feasibility (derive condition for SNCBF feasibility)
% Training (Loss function design)
% Based on theroetical foundation, we design the loss function to guide SNCBF to converge

% We generate with $b_{\theta}(x)$ with sensor noise and under different fault patterns. 

% Theorem to define a valid SCBF for polyCBF and NCBF
In this subsection, we describe how to synthesize NCBFs. 
We first present the necessary and sufficient conditions for stochastic control barrier functions, among which NCBFs constitute a special class represented by neural networks. 
% The safety of a stochastic system can be ensured safe by Theorem \ref{theorem:SCBF} given a function $b(x)$. In what follows, we shows criterion for SCBF candidates. 
% Let the estimation error to be represented as $z_t = (x_t-\hat{x}_t)$. 
% The following proposition gives the  necessary and sufficient conditions for a function $b$ to be a SCBF.  
\begin{proposition}
\label{prop:verify_scbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $b(\hat{x})$ is a stochastic control barrier function if and only if there is no $\hat{x}\in \mathcal{D}^{\gamma}:=\{\hat{x}\mid \hat{b}(\hat{x})\geq 0\}$, satisfying
$\frac{\partial b}{\partial x}g(\hat{x}) = 0$ and $\xi^\gamma(\hat{x}) < 0$, where 
\begin{multline}
\label{eq:prop2cond}
    \xi^\gamma(\hat{x}) =  \frac{\partial b}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K_{t}^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x})K_{t}\nu\right)  \\
    -\gamma||\frac{\partial b}{\partial x}(\hat{x})K_{t}c||_{2} +  \hat{b}^\gamma(\hat{x}).
\end{multline}
\end{proposition}
The proposition is based on \cite[Proposition 2]{zhang2022safe}. We omit the proof due to space constraint. 

We note that the class of NCBFs is a special subset of stochastic control barrier functions in Proposition \ref{prop:verify_scbf}. 
We denote the NCBF as $b_\theta(\hat{x})$, where $\theta$ is the parameter of the neural network representing the function. 
% We further let  $\hat{b}_\theta^\gamma(\hat{x}) = b_\theta(\hat{x}) - \Bar{b}_\theta^\gamma$ and $\Bar{b}_\theta^\gamma = \sup_{\hat{x},\hat{x}^{0}}{\{b_\theta(\hat{x}) : ||\hat{x}-\hat{x}^{0}||_{2} \leq \gamma \text{ and } b_\theta(\hat{x}^{0})=0\}}.$
% We further define
% $\mathcal{D}_\theta=\{\hat{x}|b_\theta(\hat{x})\geq 0\}$ and 
% $\mathcal{D}_\theta^\gamma=\{\hat{x}|\hat{b}_\theta^\gamma(\hat{x})\geq 0\}$.

In the following, we introduce the concept of \emph{valid} NCBFs, and present how to synthesize them. 
A valid NCBF needs to satisfy the following two properties.
\begin{definition}[Correct NCBFs]
    \label{def:correctness}
    Given a safety region $\mathcal{C}$, the NCBF $b_{\theta}$ is correct if and only if $\mathcal{D}_{\theta}:=\{\hat{x}|b_\theta(\hat{x})\geq 0\}\subseteq \mathcal{C}$. 
\end{definition}
The correctness property in Definition \ref{def:correctness} requires the NCBF $b_\theta$ to induce a set $\mathcal{D}_\theta\subseteq \mathcal{C}$.
Therefore, if the set $\mathcal{D}_\theta$ is positive invariant, then $\mathcal{C}$ is also positive invariant, and thus the robotic system is safe with respect to $\mathcal{C}$.
We next give the second property of valid NCBFs.
\begin{definition}[Feasible NCBF]
\label{def:feasibility_scbf}
    The NCBF $b_\theta$ parameterized by $\theta$ is feasible if and only if $\forall \hat{x}\in \mathcal{D}_\theta^{\gamma}:=\{\hat{x}|\hat{b}_\theta^\gamma(\hat{x})\geq 0\}$, there exists $ u$ such that $\xi_\theta^\gamma(\hat{x}) + \frac{\partial b_\theta}{\partial x}g(\hat{x})u\geq 0$, where
    \begin{multline} \label{eq:prop2cond-2}
    \xi_\theta^\gamma(\hat{x}) =  \frac{\partial b_\theta}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K_{t}^{T}\frac{\partial^{2}b_\theta}{\partial x^{2}}(\hat{x})K_{t}\nu\right)  \\
    -\gamma||\frac{\partial b_\theta}{\partial x}(\hat{x})K_{t}c||_{2} +  \hat{b}_\theta^\gamma(\hat{x}).
\end{multline}
\end{definition}
The feasibility property in Definition \ref{def:feasibility_scbf} ensures that a control input $u$ can always be found to satisfy the inequality \eqref{eq:SCBF-2}, and hence can guarantee safety.
% Based on Proposition \ref{prop:verify_scbf} and Definition \ref{def:feasibility}, feasible SNCBFs can be defined as follows. 

% \begin{definition}[Feasible SNCBF]
% \label{def:feasibility_scbf}
%     The SNCBF $b_\theta$ parameterized by $\theta$ is feasible if and only if $\forall \hat{x}\in \mathcal{D}^{\gamma}$, $\exists u$ s.t. $\xi(\hat{x}) + \frac{\partial b_\theta}{\partial x}g(\hat{x})u\geq 0$. 
% \end{definition}

% Besides the feasibility property given in Definition \ref{def:feasibility_scbf}, a valid SNCBF $b_\theta$ also needs to be correct as shown in Definition \ref{def:correctness}. 
We note that there may exist infinitely many valid NCBFs. 
In this work, we focus on synthesizing valid NCBFs that encompass the largest possible safety region. To this end, we define an operator $Vol(\mathcal{D}_\theta)$ to represent the volume of the set $\mathcal{D}_\theta$, and synthesize a valid NCBF such that $Vol(\mathcal{D}_\theta)$ is maximized. The optimization program is given as follows
\begin{align}
    \label{eq:train_obj}
    \max_{\theta}&\quad{Vol(\mathcal{D}_\theta)} \\
    \label{eq:train_feasible_cons}
    s.t. & \quad \xi_\theta^\gamma(\hat{x}) \geq 0 \quad \forall \hat{x}\in \partial \mathcal{D}_\theta^{\gamma} \\
    \label{eq:train_correct_cons}
    & \quad b_{\theta}(\hat{x}) \leq h(\hat{x}) \quad \forall \hat{x}\in \mathcal{X}\backslash\mathcal{D}_\theta
\end{align}
% where $\mathcal{D}^\gamma:=\{\hat{x}\mid \hat{b}^{\gamma}_{\theta}(\hat{x})\geq 0\}$. 
Here constraints \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} require parameter $\theta$ to define feasible and correct NCBFs, respectively.
% In what follows, we refer to \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} as feasibility and correctness constraints.
Solving the constrained optimization problem is challenging. In this work, we convert the constrained optimization to an unconstrained one by constructing a loss function which penalizes violations of the constraints.
We then minimize the loss function over a training dataset to learn parameters $\theta$ and thus NCBF $b_\theta$.
% A valid SNCBF is feasible as defined in Definition \ref{def:feasibility_scbf} and is correct defined in Definition \ref{def:correctness}. 
% Besides, a good SNCBF should not only be valid but also cover as much safe region as possible. We define an operator $Vol(\mathcal{D}_\gamma)$ represent the volume of the set $\mathcal{D}^{\gamma}$.  We next demonstrate how to synthesize a valid SNCBF. 
% To ensure the synthesized SCBF, we proposed the following loss function
% loss function design goes here

We denote the training dataset as $\mathcal{T}:=\{\hat{x}_{1}, \ldots, \hat{x}_{N}\mid \hat{x}_{i}
\in \mathcal{X}, \forall i =1,\ldots,N\}$, where $N$ is the number of samples. The dataset $\mathcal{T}$ is generated by simulating estimates with fixed point sampling as in \cite{dawson2023safe}. We first uniformly discretize the state space into cells with length vector $L$. Next, we uniformly sample the center of discretized cell as fixed points $x_{f}$. Then we simulate the estimates by introducing a perturbation $\rho[j]$  sampled uniformly from interval $[x_{f}[j]-0.5 L[j], x_{f}[j]+0.5 L[j]]$. Finally, we have the sampling data $\hat{x}_i=x_{f}+\rho\in \mathcal{T}\subseteq \mathcal{X}$.
% The estimates $x_{R}$ are synthesized with $x_{f}$ perturbed by Gaussian noise, i.e., $x_{R}[j] = x_{f}[j] + \mathcal{N}(0, \sigma_{j}^2)$ where $\sigma_{j}$ is the standard deviation of corresponding sensor indexed $j$.

% Then a valid SNCBF can be trained using $\mathcal{T}$ by solving the following optimization program. 
% %The training of SNCBF can be summarized as a constrained optimization problem as follows. 
% \begin{align}
%     \label{eq:train_obj}
%     \max_{\theta}&\quad{Vol(\mathcal{D}^\gamma)} \\
%     \label{eq:train_feasible_cons}
%     s.t. & \quad \xi(\hat{x}) \geq 0 \quad \forall \hat{x}\in \partial \mathcal{D}^{\gamma} \\
%     \label{eq:train_correct_cons}
%     & \quad \hat{b}_{\theta}(\hat{x}) \leq h(\hat{x}) \quad \forall \hat{x}\in \mathcal{X}\backslash\mathcal{D}^{\gamma}
% \end{align}
% where $\mathcal{D}^\gamma:=\{\hat{x}\mid \hat{b}^{\gamma}_{\theta}(\hat{x})\geq 0\}$. 
% Here constraints \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} require parameter $\theta$ to define feasible and correct SNCBFs, respectively.
% In what follows, we refer to \eqref{eq:train_feasible_cons} and \eqref{eq:train_correct_cons} as feasibility and correct constraints.
% Solving the constrained optimization problem is challenging. In this work, we convert the constrained optimization to an unconstrained one using the Lagrangian method \cite{hestenes1969multiplier}, which introduces a Lagrangian multiplier to penalize violations of the constraints. 
We then formulate the following unconstrained optimization problem to search for $\theta$
\begin{equation}
    \label{eq:uncons_opt}
    \min_{\theta}\quad{-Vol(\mathcal{D}_{\theta})} + \lambda_{f}\mathcal{L}_f + \lambda_{c}\mathcal{L}_c 
\end{equation}
where $\mathcal{L}_f$ is the loss penalizing the violations of constraint \eqref{eq:train_feasible_cons}, $\mathcal{L}_c$ penalizes the violations of constraint \eqref{eq:train_correct_cons}, and $\lambda_{f}$ and $\lambda_{c}$ are non-negative coefficients. 
The objective function \eqref{eq:train_obj} is approximated by the following quantity
\begin{equation}
    \label{eq:volume_obj}
    Vol(\mathcal{D}_{\theta}) = \sum_{\hat{x}\in \mathcal{T}}{-ReLU(h(\hat{x}))ReLU(-b_{\theta}(\hat{x}))}. 
\end{equation}
The idea is to penalize samples $\hat{x}$ in the safety region but not in $\mathcal{D}_\theta$, i.e., $h(\hat{x})>0$ and $b_\theta(\hat{x})<0$. 
The penalty of violating the feasibility property in Eq. \eqref{eq:train_feasible_cons} is defined as
\begin{equation}\label{eq:Lf-SNCBF}
    \mathcal{L}_f = \sum_{\hat{x}\in \mathcal{T}} -\Delta(\hat{x}) ReLU(-\xi_\theta^\gamma(\hat{x}) - \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u + \hat{b}^\gamma_\theta(\hat{x})), 
\end{equation}
where $\Delta(\hat{x})$ is an indicator function such that $\Delta(\hat{x}):= 1$ if $b_{\theta}(\hat{x})=\overline{b}^{\gamma}_\theta$ and $\Delta(\hat{x}):= 0$ otherwise. The function $\Delta$ allows us to find and penalize sample points $\hat{x}$ satisfying $\hat{b}_{\theta}^\gamma(\hat{x})=0$ and  $\xi_\theta^\gamma(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u <0 $.
% We penalize for the points that the following two condition hold
% \begin{enumerate}
%     \item $b_{\theta}(\hat{x})=0$.
%     \item $\xi(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u <0 $. 
% \end{enumerate}
For each sample $\hat{x}\in\mathcal{T}$, the control input $u$ in Eq. \eqref{eq:Lf-SNCBF} is computed as follows 
\begin{equation}
\begin{split}
    \min_{u} & \quad u^{T}u \\
    s.t. & \quad \xi_\theta^\gamma(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u \geq 0
\end{split}
\end{equation}
The loss function to penalize the violations of the correctness property in Eq. \eqref{eq:train_correct_cons} is constructed as 
\begin{equation}
    \label{eq:correctness_loss}
    \mathcal{L}_c = \sum_{\hat{x}\in \mathcal{T}}{ReLU(-h(\hat{x}))ReLU(b_{\theta}(\hat{x}))}
\end{equation}
The term $\mathcal{L}_c$ penalizes the samples $\hat{x}$ outside the safety region but being regarded safe, i.e., $h(\hat{x})<0$ and $b_{\theta}(\hat{x})>0$. 
When $\mathcal{L}_c$ and $\mathcal{L}_f$ converge to $0$, constraints \eqref{eq:train_feasible_cons}-\eqref{eq:train_correct_cons} are satisfied.
% The proposed framework can either train a bank of SNCBF or a solo SNCBF that can further be used for safety constraint construction. 


\subsection{Synthesis of FT-NCBF}\label{sec:FT-NCBF}
% Synthesis of FT-SNCBF 
% Fault-tolerent is an extension of SNCBF
% conclude what we have in previous section and introduce what we are going to have in this section
% In the previous subsection, we described how to learn SNCBFs from data. 
In Section \ref{sec:SNCBF}, we presented the training of NCBFs when there exists no adversary.
In this subsection, we generalize the construction of the loss function Eq. \eqref{eq:uncons_opt}, and present how to train a valid FT-NCBF for robotic systems in Eq. \eqref{eq:state-sde}-\eqref{eq:output-sde} under unknown attack patterns.
With a slight abuse of notations, we use $b_\theta$ to denote the FT-NCBF in the remainder of this paper. 
% Notations $\hat{b}_\theta^\gamma(\hat{x})$, $\Bar{b}_\theta^\gamma$, $\mathcal{D}_\theta$, and  $\mathcal{D}_\theta^\gamma$ are defined in a similar fashion as we did in Section \ref{sec:SNCBF}.
% Specifically, we desire a function $b_{\theta}$ to satisfy the properties defined in Definition \ref{def:feasibility_scbf} and \ref{def:correctness}. 
% Based on the generalized properties, we next formulate a loss function to train a valid fault tolerant-SNCBF (FT-SNCBF) for all fault patterns.
We define $\hat{b}_\theta^{\gamma_i}(\hat{x})=b_\theta(\hat{x})-\Bar{b}_\theta^{\gamma_i}(\hat{x})$, where
\begin{equation*}
\overline{b}_{\theta}^{\gamma_{i}}
= \sup_{\hat{x},\hat{x}^{0}}{\left\{b_{\theta}(\hat{x}) : ||\hat{x}-\hat{x}^{0}||_{2} \leq \gamma_{i}\right.} \\
\left. \text{ and } b_{\theta}(\hat{x}^{0})=0\right\}.
\end{equation*}
%We further let $\mathcal{D}_\theta^{\gamma_i}=\{\hat{x}\mid \hat{b}_\theta^{\gamma_i}(\hat{x})\geq 0\}$.
The following proposition gives the  necessary and sufficient conditions for a function $b_{\theta}$ to be an FT-NCBF.  

\begin{proposition}
\label{prop:verify_ftscbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $b_{\theta}(\hat{x})$ is an FT-NCBF if and only if there is no $\hat{x}\in \mathcal{D}_\theta^{\gamma_i}$, satisfying
$\frac{\partial b_\theta}{\partial x}g(\hat{x}) = 0$ , $\xi_\theta^{\gamma_i}(\hat{x}) < 0$ for all $i\in \{1,\ldots,m\}$ where 
\begin{multline}
\label{eq:ftsncbf_cond}
    \xi_\theta^{\gamma_i}(\hat{x}) =  \frac{\partial b_\theta}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}b_\theta}{\partial x^{2}}(\hat{x})K\nu\right) + \\
    ||\frac{\partial h}{\partial x}(\hat{x})K_{t,i}c||_{2} +  \hat{b}^{\gamma_i}_\theta(\hat{x}).
\end{multline}
\end{proposition}
The proposition can be proved using the similar idea to Proposition \ref{prop:verify_scbf}. We omit the proof due to space constraint. 

We construct the following loss function to learn the FT-NCBF 
\begin{equation}
    \label{eq:train_ftsncbf}
    \min_{\theta}\quad{-Vol(\mathcal{D}_{\theta})} + \lambda_f\sum_{i\in \{1,\ldots,m\}}{\mathcal{L}^{i}_{f}} + \lambda_c\mathcal{L}_c, 
\end{equation}
% We define the objective function as \eqref{eq:volume_obj} and the correctness constraint as \eqref{eq:correctness_loss}. 
where $\mathcal{L}_{f} = \sum_{i\in \{1,\ldots,m\}}{\mathcal{L}^{i}_{f}}$ is the penalty of violating the feasibility property,
\begin{equation*}
    \mathcal{L}^{i}_{f} = \sum_{\hat{x}\in \mathcal{T}} -\overline{\Delta}_{i}(\hat{x}) ReLU(-\xi_\theta^{\gamma_i}(\hat{x}) - \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u + \hat{b}_\theta^{\gamma_i}(\hat{x})), 
\end{equation*}
and $\overline{\Delta}(\hat{x})$ is an indicator function such that $\overline{\Delta}(\hat{x}):= 1$ if $b_{\theta}(\hat{x})\leq\max_{i\in Z_t}{\{\overline{b}^{\gamma_i}_\theta\}}$ and $\overline{\Delta}(\hat{x}):= 0$ otherwise. 
The control input $u$ used to compute $\mathcal{L}_f^i$ for each sample $\hat{x}$ is calculated as follows. 
\begin{equation}
\label{eq:ctrl_multiSNCBF}
\begin{split}
    \min_{u} & \quad u^{T}u \\
    s.t. & \quad \xi_\theta^{\gamma_i}(\hat{x}) + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u \geq 0 \quad \forall i\in \{1,\ldots,m\}
\end{split}
\end{equation}
When $\mathcal{L}_c$ and $\mathcal{L}_f$ converge to $0$, the learned $b_{\theta}$ is a valid FT-NCBF. 
% Note that a good SNCBF candidate does not guarantee valid. The verification of a SNCBF candidate is needed and is a non-trivial process. 

\subsection{Safety-Critical Control Synthesis using FT-NCBF}\label{sec:conflict}
% FT-Framework (Controller synthesis)
% EKF banks FT-framework
% Safety guarantee
% A training procedure is proposed in previous sections for SNCBF and FT-SNCBF. However, to ensure safety of a system, a fault-tolerant framework for safe control in non-trivial. Hence, we address this issue in this subsection. 


In Section \ref{sec:FT-NCBF}, we discussed how to train an FT-NCBF. 
In this subsection, we describe how to utilize the learned FT-NCBF to synthesize control policies for robots under sensor faults and attacks to guarantee safety.

% We first employ an EKF to compute state estimates using all sensor measurements $\{1,\ldots,q\}$.
We maintain a set of EKFs to compute state estimates.
Each EKF is associated with the sensor measurements from $\{1,\ldots,q\}\setminus \mathcal{F}(r_i)$ for all $i=1,\ldots,m$, i.e., measurements obtained by excluding $\mathcal{F}(r_i)$.
We denote the state estimates obtained after excluding sensors associated with attack pattern $r_i$ as $\hat{x}_{t,i}$.
We define 
\begin{equation*}
    \Omega_i = \{u:\xi_\theta^{\gamma_i} + \frac{\partial b_{\theta}}{\partial x}g(\hat{x}) u \geq 0\}
\end{equation*}
as the feasible region when searching for control input under attack pattern $r_i$
Then if there exists a control input $u\in\cap_{i=1}^m\Omega_i\neq\emptyset$, such a control input can guarantee the safety under any attack pattern $r_i$.

We note that the existence of a control input $u$ satisfying the constraints specified by $\Omega_i,\ldots,\Omega_m$ simultaneously may not be guaranteed because sensor faults and attacks can significantly bias the state estimates.
Thus we develop a mechanism to identify constraints conflicting with each other, and resolve such conflicts.
Our idea is to additionally maintain ${m \choose 2}$ EKFs, where each EKF computes state estimates using sensors from $\{1,\ldots,q\}\setminus(\mathcal{F}(r_i)\cup\mathcal{F}(r_j))$ for all $i\neq j$.
We use a variable $Z_t$ to keep track of the attack patterns that will not raise conflicts.
The variable $Z_t$ is initialized as $\{1,\ldots,m\}$.
If $\cap_{i\in Z_t}\Omega_i=\emptyset$, we compare state estimates $\hat{x}_{t,i}$ with $\hat{x}_{t,j}$ for all $i,j\in Z_t$ and $i\neq j$.
If $\|\hat{x}_{t,i}-\hat{x}_{t,j}\|_2\geq \alpha_{ij}$ for some chosen parameter $\alpha_{ij}>0$, then $Z_t$ is updated as 
\begin{equation*}
    Z_t = \begin{cases}
        Z_t\setminus \{i\},&\mbox{ if }\|\hat{x}_{t,i}-\hat{x}_{t,i,j}\|_2\geq \alpha_{ij}/2\\
        Z_t\setminus \{j\},&\mbox{ if }\|\hat{x}_{t,j}-\hat{x}_{t,i,j}\|_2\geq \alpha_{ij}/2
    \end{cases}.
\end{equation*}
After updating $Z_t$, if $\cap_{i\in Z_t}\Omega_i\neq\emptyset$, then control input $u_t$ can be chosen as
\begin{equation}\label{eq:control synthesis}
    \min_{u_t\in\cap_{i\in Z_t}\Omega_i}~u_t^Tu_t.
\end{equation}
Otherwise, we will remove indices $i$ corresponding to attack pattern $r_i$ that leads to largest residue $\Bar{y}_{t,i}-\Bar{c}_i\hat{x}_{t,i}$ until $\cap_{i\in Z_t}\Omega_i\neq \emptyset$.
Here $\Bar{y}_{t,i}$ is the output from sensors in $\{1,\ldots,q\}\setminus \mathcal{F}(r_i)$.

We summarize the procedure for synthesizing control inputs using FT-NCBF in Algorithm \ref{alg:ftcontrol}. 
In what follows, we present the safety guarantee of our approach.

% In this subsection, we develop a fault tolerant framework which utilizes the learned FT-SNCBF to synthesize a control policy to guarantee safety.
% We maintain $1+m+{m \choose 2}$ EKFs.
% \begin{enumerate}
%     \item $1$: One EKF is designed for fault free case. 
%     \item $m$: Each EKF corresponds to a different possible fault pattern in $\{r_1,\dots r_m\}$. 
%     \item ${m \choose 2}$: Each EKF corresponds to the combination of fault pattern $i,j\in\{r_1,\dots r_m\}$, $i\neq j$. 
% \end{enumerate}
% We ensure safety with probability $(1-\epsilon)$ by synthesizing a FT-SNCBF and construct $m+1$ corresponding constraints for each fault pattern on the control input. The deployment of the proposed FT-Framework can be summarized in the following Algorithm.
\begin{algorithm}[h]
\begin{algorithmic}[]
\caption{Safety-Critical Control Synthesis using FT-NCBF}\label{alg:ftcontrol}
    \State \textbf{Input:} Sensor measurements $y_{t}$, collection of attack patterns $r_1,\ldots,r_m$, learned FT-NCBF $b_{\theta}$
    \State \textbf{Output:} Control Input $u_t$
    % \Procedure{$u = FTC$}{$y_{t}\mid \mathcal{F}, b_{\theta}$}
    % \State $\hat{x}_{t} \leftarrow EKF(y_{t})$
        \State $\hat{x}_{t,i} \leftarrow EKF(\Bar{y}_{t,i})$ for all $i\in \{1,\dots,m\}$
        \State $\hat{x}_{t,i,j} \leftarrow EKF(\Bar{y}_{t,i,j})$ for all $i,j \in \{1,\dots,m\}$ and $i\neq j$
    \State $Z_{t} \leftarrow \{1, \dots, m\}$
    \While {$\cap_{i\in Z_t}\Omega_i=\emptyset$}
    \For{$i,j \in Z_t$ such that $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} > \alpha_{ij}$} 
        \If{$||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} > \alpha_{ij}/2$}
            \State $Z_{t} \leftarrow Z_{t} \setminus \{i\}$
        \ElsIf{$||\hat{x}_{t,j}-\hat{x}_{t,i,j}||_{2} > \alpha_{ij}/2$}
            \State $Z_{t} \leftarrow Z_{t} \setminus \{j\}$
        \EndIf
    \EndFor
    \If{$\bigcap_{i \in Z_{t}}{\Omega_{i}} \neq \emptyset$}
            \State Compute $u_t$ using Eq. \eqref{eq:control synthesis}
            \State \textbf{Return $u_t$}
    \Else
    \State $i_{r} \leftarrow \arg\max_{i}{\{\overline{y}_{t,i}-\overline{c}_{i}\hat{x}_{t,i}\}}$. 
    \State $Z_{t} \leftarrow Z_t\setminus\{i_{r}\}$.
    \EndIf
    \EndWhile
    % \EndProcedure
\end{algorithmic}
\end{algorithm}

We next show the safety guarantee of the system under sensor faults. The following result gives the sufficient conditions of safety. 
\begin{lemma}[\cite{clark2020control}]
    \label{lemma:ftsafe}
    Suppose  $\gamma_{1},\ldots,\gamma_{m}$, and $\alpha_{ij}$ for $i < j$ are chosen such that the following conditions are satisfied:
    \begin{enumerate}
    \item Define  $\Lambda_{i}(\hat{x}_{t,i}) = \frac{\partial b_\theta^{\gamma_i}}{\partial x}g(\hat{x}_{t,i})$. There exists $\delta > 0$ such that for any $X_{t}^{\prime} \subseteq X_{t}(\delta):=\{i\mid \hat{b}_{\theta}^{\gamma_i}(\hat{x}_{t,i})<\delta\}$ satisfying $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} \leq \alpha_{ij}$ for all $i,j \in X_{t}^{\prime}$,  there exists $u$ such that
    \begin{equation}
    \label{eq:FT-CBF2}
    \Lambda_{i}(\hat{x}_{t,i})u > -\xi_\theta^{\gamma_i}
    \end{equation}
    for all $i \in Z_t$.
    \item For each $i$, when $r=r_{i}$, 
    \begin{multline}
    \label{eq:FT-CBF3}
    Pr(||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \alpha_{ij}/2 \ \forall j, ||\hat{x}_{t,i}-x_{t}||_{2} \leq \gamma_{i} \ \forall t)\\
     \geq 1-\epsilon.
    \end{multline}
    \end{enumerate}
    Then $Pr(x_{t} \in \mathcal{D}_\theta \ \forall t) \geq 1-\epsilon$ for any attack pattern $r \in \{r_{1},\ldots,r_{m}\}$.
\end{lemma}
However, Lemma \ref{lemma:ftsafe} depends on the existence of $u_{t}$. The following proposition provides sufficient condition of the existence of $u_{t}$ for all $\hat{x}\in \mathcal{D}^{\gamma_i}_{\theta}, \ \forall i\in Z_{t}$.  
\begin{proposition}
    \label{prop:u_f_ftsncbf}
    Suppose an FT-NCBF $b_{\theta}$ makes losses $\mathcal{L}_f+\mathcal{L}_c\rightarrow 0$ as the training dataset $\mathcal{T}$ approaches $\mathcal{X}$.
    Then, there always exists $u_{t}$ such that $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})u_{t}+\xi_\theta^{\gamma_i}\geq 0$ $\forall \hat{x}\in \mathcal{D}_{\theta}^{\gamma_i}, \ \forall i\in Z_t$. 
\end{proposition}
\begin{proof}
    By the constructions of $\mathcal{L}_f^i$ and $\mathcal{L}_c$, we first note that these losses are non-negative. Thus if $\mathcal{L}_f+\mathcal{L}_c\rightarrow 0$, we must have that $\mathcal{L}_f^i,\mathcal{L}_f,\mathcal{L}_c\rightarrow 0$.
    According to the definitions of $\mathcal{L}_f$ and $\mathcal{L}_f^i$, we then have that there must exist some control input $u$ that solves the optimization program in Eq. \eqref{eq:ctrl_multiSNCBF} when  $\mathcal{L}_f^i,\mathcal{L}_f\rightarrow 0$. Otherwise losses $\mathcal{L}_f^i$ and $\mathcal{L}_f$ will be positive.
\end{proof}
% \begin{proposition}
%     \label{prop:u_f_ftsncbf}
%     Suppose a FT-SNCBF $b_{\theta}$ satisfies the conditions in Proposition \ref{prop:verify_ftscbf} for $i\in Z_{t}$. Then, there always exists $u_{t}$ such that $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})u_{t}+\xi_{i}\geq 0$ $\forall \hat{x}\in \mathcal{D}_{\theta}^{\gamma_i}, \ \forall i\in Z_t$. 
% \end{proposition}
% \begin{proof}    
%     We prove by showing there always exists $u_t$ such that \eqref{eq:SCBF-2} hold for two cases, namely, (i) $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})\neq0$ and (ii) $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})=0$. 
%     For case (ii), we can always choose $u_{t}$ such that \eqref{eq:SCBF-2} holds for all $i\in Z_t$. For case (ii), there does not exist $\hat{x}$ such that $\frac{\partial b_{\theta}}{\partial x}g(\hat{x})=0$ and $\xi_i(\hat{x})< 0$ by Proposition \ref{prop:verify_ftscbf}. Hence, $u_{t}$ can be any real value. 
% \end{proof}
We finally conclude this section by presenting the safety guarantee provided by our approach. 
\begin{theorem}[Safety Guarantee under Sensor Faults]
    \label{th:FT_Safety}
    Let $b_{\theta}$ be an FT-NCBF such that $\mathcal{L}_f+\mathcal{L}_c\rightarrow 0$ as the training dataset $\mathcal{T}$ approaches $\mathcal{X}$. 
    Suppose $\gamma_{1},\ldots,\gamma_{m}$, and $\alpha_{ij}$ for $i < j$ are chosen such that the conditions in Lemma \ref{lemma:ftsafe} hold. Then $Pr(x_{t} \in \mathcal{D} \ \forall t) \geq 1-\epsilon$ for any attack pattern $r \in \{r_{1},\ldots,r_{m}\}$. 
\end{theorem}
\begin{proof}
    The theorem immediately follows from Lemma \ref{lemma:ftsafe} and Proposition \ref{prop:u_f_ftsncbf}.
\end{proof}
% \begin{theorem}[Safety Guarantee under Sensor Faults]
%     \label{th:FT_Safety}
%     Given an FT-SNCBF $b_{\theta}$ satisfies the conditions in Proposition \ref{prop:verify_ftscbf} for $i\in Z_{t}$. Suppose $\gamma_{1},\ldots,\gamma_{m}$, and $\theta_{ij}$ for $i < j$ are chosen such that conditions in \ref{lemma:ftsafe} hold. Then $Pr(x_{t} \in \mathcal{D} \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$. 
% \end{theorem}
% \begin{proof}
%     By \cite[Theorem 3]{clark2020control} if there exist $u_{t}$ such that $\Omega_{i}$ holds 
%     $\forall \hat{x}\in \mathcal{D}^{\gamma}_{\theta}$ $\forall i\in Z_{t}$ then, by Theorem \ref{theorem:SCBF}, 
%     \begin{multline*}
%     Pr(x_{t} \in \mathcal{D} \ \forall t | ||\hat{x}_{t,i}-\hat{x}_{t}||_{2} \leq \gamma_{i}, \\ ||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \theta_{ij}/2 \ \forall t) = 1
%     \end{multline*}
%     By Proposition \ref{prop:u_f_ftsncbf}, there exist $u_t$ s.t. $\Omega_{i}$ holds for all $\hat{x}\in \mathcal{D}^{\gamma_i}\quad \forall i\in Z_{t}$. 
%     and $Pr(x_{t} \in \mathcal{D}\subseteq \mathcal{C} \ \forall t) > 1-\epsilon$ by (\ref{eq:FT-CBF3}).
% \end{proof} 

% \subsection{FT-NCBF Design}
% The network is designed to take all estimates $\hat{x}_i$, $\forall i$ and indicator $I$. Intuitively, the indicator works like a mask to filter out unwanted estimates and activate different gain for corresponding $\gamma_i$

% \subsection{EKF Residual-based Fault Pattern Classification (Potential)}
% \textbf{Action needed **} The classification requires us to derive a guarantee. Fundamentally, the classifier is to make the whole design of the framework more cohesive by removing step 1, 2 and 3. 


==> sections/Intro.tex <==
\section{INTRODUCTION}

Robotic systems are increasingly deployed in safety-critical applications such as search and rescue in hazardous environments. \cite{fernandez2023distributed,peng2023safe,jian2023dynamic}. 
Safety requirements are normally formulated as the forward invariance property of a given safety regionm.
Violations of safety could lead to catastrophic damages to robots, hurt to humans that co-exist in the field of activities, and economic loss \cite{knight2002safety,schwarting2018planning}.
%Various approaches have been proposed to guarantee safety, including HJ reachability-based approach \cite{bansal2017hamilton,choi2021robust} and safe reinforcement learning \cite{brunke2022safe,westenbroek2021combining,chow2019lyapunov}. 
An emerging class of methods for safety-critical synthesis is control barrier function (CBF)-based approaches \cite{ames2019control,xu2015robustness,Wei2021high,tan2021high}.
These approaches induce a quadratic program for safety-critical control synthesis of nonlinear control-affine systems.
However, such approaches become invalid when the robotic systems are subject to sensor faults or attacks.

Robotic systems utilize sensor measurements to estimate their states, and further calculate control signals to satisfy safety constraints.
However, sensors are shown to be vulnerable to a wide range of faults and malicious attacks, making safety-critical control challenging in such scenarios \cite{mo2010false,guan2017distributed}. 
When sensors are under faults or attacks, robotic systems obtain biased state estimates, leading to erroneous control inputs.
CBF-based safety-critical synthesis for autonomous systems with incomplete information was firstly investigated in \cite{clark2019control}, and is later extended in \cite{clark2020control} to tolerate sensor faults and attacks. 

Safety-critical synthesis employing CBF-based approaches implicitly assume that the CBF is known.
Such an assumption, however, may not always hold in practice \cite{srinivasan2020synthesis}.
CBF synthesis is investigated to bridge this gap.
For robotic systems with polynomial dynamics, CBF synthesis is formulated as sum-of-squares (SOS) optimization programs \cite{clark2021verification,clark2022semi,kang2023verification,dai2022convex,jagtap2020formal}.
These SOS-based approaches, however, does not scale to high-dimensional systems with complex system dynamics, e.g., learning-enabled robotic systems \cite{tampuu2020survey} and neural network dynamical models \cite{raissi2019physics,gamboa2017deep}, which significantly limits the applicability of CBF-based safety-critical control \cite{kojima2005sparsity}.

To overcome the shortcomings of CBF synthesis using SOS-based approaches, neural control barrier functions (NCBFs) \cite{dawson2022safe,dawson2023safe,liu2023safe}, which represent CBFs using neural networks, are developed.
NCBFs leverage the universal approximation power of neural networks \cite{tabuada2022universal,hornik1989multilayer,csaji2001approximation}, facilitating the CBF synthesis and thus enabling safety-critical control of high-dimensional complex systems through the application of machine learning techniques \cite{srinivasan2020synthesis,xiao2021barriernet,dawson2023safe,dawson2022learning,robey2020learning,lindemann2021learning}.
These approaches, however, are not applicable in the presence of sensor faults and attacks.

In this paper, we study the synthesis of stochastic neural CBFs (SNCBFs) and the corresponding safety-critical control of robotic systems under sensor faults and attacks.
We consider that an adversary can choose an arbitrary fault or attack pattern among finitely many choices, where each pattern corresponds to a distinct subset of compromised sensors.
We employ a set of extended Kalman filters (EKFs) to estimate the system states.
Each EKF is associated with the sensor measurements obtained by excluding the sensors within one pattern.
To address sensor faults and attacks, we propose a class of fault-tolerant SNCBFs (FT-SNCBFs).
We present a data-driven approach to learn FT-SNCBFs.
% We develop the necessary and sufficient conditions for a function to be a FT-SNCBF.
% We then construct a loss function which penalizes any violation of our derived conditions to train a FT-SNCBF using the state estimation from each EKF.
The learned FT-SNCBFs are then integrated into a quadratic program for safety-critical control synthesis. 
If some control input can be found, then such an input can guarantee the safety constraint regardless of the faults and attacks.
If no control input can be found, it indicates that there exist conflicting FT-SNCBFs, yielding empty solution space for the problem safety-critical control synthesis.
We develop a conflict resolution mechanism to resolve such scenarios.
To summarize, this paper makes the following contributions.
\begin{itemize}
    \item We propose FT-SNCBFs to guarantee the safety of stochastic robotic systems under sensor faults and attacks. We derive the necessary and sufficient conditions for a function to be a valid FT-SNCBF.
    We construct a loss function using our derived conditions to learn FT-SNCBFs from data.
    \item We develop a fault-tolerant framework which utilizes our proposed FT-SNCBFs for safety-critical control synthesis. The framework resolves conflicts between multiple FT-SNCBFs. Specifically, we compare the state estimates of each conflicting pattern with a baseline, where state estimate is obtained by excluding all sensor measurements from conflicting patterns.
    If the comparison exceeds a threshold, then the sensor measurements are likely compromised by faults or attacks, and thus should be ignored.
    % \item We propose stochastic NCBFs to guarantee the safety of stochastic robotic systems in the absence of faults and attacks. We derive the necessary and sufficient conditions for a function to be a valid stochastic NCBF.
    % We craft a loss function using our derived conditions to train SNCBFs.
    % \item We generalize the concept of stochastic NCBFs to FT-SNCBFs to mitigate sensor faults and attacks. 
    \item We evaluate our approach using a case study. We show that our proposed approach guarantees the robot to satisfy the safety constraint regardless of the faults and attacks, whereas the baseline employing the existing neural CBF-based approach fails.
\end{itemize}

The rest of this paper is organized as follows. 
Section \ref{sec:formulation} presents preliminaries and problem formulation.
We synthesize the FT-SNCBFs, and utilize them for safety-critical control in Section \ref{sec:sol}.
Our developed approach is demonstrated in Section \ref{sec:exp}.
Section \ref{sec:conclusion} concludes this paper.


% \subsection{Timeline}
% \begin{itemize}
%     \item Safety Counter-example (08/30)
%     \item Obs Case Study (8/30)
%     \item FTSNCBF quad training (08/31)
% \end{itemize}

% \subsection{Contributions}

% \begin{enumerate}
%     \item We propose a loss function to train a valid stochastic NCBF to ensure safety under sensor faults and attacks with desired probability.
%     \item We propose a fault-tolerant framework for Resilient NCBFs that ensures safety under sensor faults and attacks with desired probability. 
%     \item We ensure safety of the system using proposed framework under sensor faults with desired probability. 
% \end{enumerate}

% outline of technical part
% \begin{enumerate}
%     \item overall design \\
%     The overall structure of the method, providing a general overview of each component. 
%     \item SNCBF feasibility condition (extend to FT-SNCBF feasibility condition) \\
%     Introduce what condition make the SNCBFs/FT-SNCBF good ones. (Contribution 1)
%     \item SNCBF/FT-SNCBF Training Framework (loss function design) (Contribution 2)
%     \item FT-Framework (Theorem on safety guarantee) (Contribution 3)
% \end{enumerate}


==> sections/Preliminaries.tex <==
\section{Preliminaries}

We then select parameters $\gamma_{1},\ldots,\gamma_{m} \in \mathbb{R}_{+}$, and $\{\theta_{ij} : i < j\} \subseteq \mathbb{R}_{+}$, $\delta > 0$. %,  a collection of functions $B_{1},\ldots,B_{m}: \mathbb{R}^{n} \rightarrow \mathbb{R}$, and a collection of class-K functions $\alpha_{3}^{i} : i=1,\ldots,m$. 
The set of feasible control actions is defined at each time $t$ using the following steps:
\begin{enumerate}
\item Define $X_{t}(\delta) = \{i : \hat{h}_{i}(\hat{x}_{t,i}) < \delta\}$. Let $Z_{t} = X_{t}(\delta)$. Define a collection of sets $\Omega_{i}$, $i \in Z_{t}$, by  
\begin{multline}%{rCl}
%\nonumber
\Omega_{i} 
\triangleq \left\{u: \frac{\partial h_{i}}{\partial x}(\hat{x}_{t,i})\overline{f}(\hat{x}_{t,i},u_{t}) - \gamma_{i}||\frac{\partial h}{\partial x}(\hat{x}_{t,i})K_{t,i}c||_{2}\right.  \\
\label{eq:FTCBF-constraints}
 \left.+ \frac{1}{2}\mathbf{tr}(\overline{\nu}_{t,i}^{T}K_{t,i}^{T}\frac{\partial^{2}h_{i}}{\partial x^{2}}(\hat{x}_{t,i})K_{t,i}\overline{\nu}_{t,i}) \geq -\hat{h}_{i}(\hat{x}_{t,i})\right\}. %\IEEEeqnarraynumspace
\end{multline}
 Select  $u_{t}$ satisfying $u_{t} \in \bigcap_{i \in X_{t}(\delta)}{\Omega_{i}}$. If no such $u_{t}$ exists, then go to Step 2.
\item For each $i,j$ with $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} > \theta_{ij}$, set $Z_{t} = Z_{t} \setminus \{i\}$ (resp. $Z_{t} = Z_{t} \setminus \{j\}$) if $||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} > \theta_{ij}/2$ (resp. $||\hat{x}_{t,j}-\hat{x}_{t,i,j}||_{2} > \theta_{ij}/2$).
  If  $\bigcap_{i \in Z_{t}}{\Omega_{i}} \neq \emptyset$,  then select $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$. Else go to Step 3.
\item Remove the indices $i$ from $Z_{t}$ corresponding to the estimators with the largest residue values $\overline{y}_{t,i}-\overline{c}_{i}\hat{x}_{t,i}$ until there exists $u_{t} \in \bigcap_{i \in Z_{t}}{\Omega_{i}}$.
\end{enumerate}
This policy aims to select a control input that guarantees safety regardless of the fault pattern that is experienced (Step 1). If no such input exists, then the set of constraints is pruned by looking for constraints $\Omega_{i}$ such that  $\hat{x}_{t,i}$ deviates from  $\hat{x}_{t,i,j}$ by more than a threshold value, since such deviations are likely to be due to faults. Meanwhile, if the fault pattern is $r_{i}$, then the estimates $\hat{x}_{t,i}$ and $\hat{x}_{t,i,j}$ will likely be close to one another for all $t$ and $j \neq i$, since both estimators do not rely on the faulted sensor. We note that these constraints are compatible with feedback policies as well as more general history-based control policies. 

\begin{theorem}
\label{theorem:FT-CBF}
Define 
\begin{multline*}
\overline{h}_{\gamma_{i}} 
= \sup{\left\{h(x) : ||x-x^{0}||_{2} \leq \gamma_{i}\right.} \\
\left. \mbox{ for some } x^{0} \in h^{-1}(\{0\})\right\}
\end{multline*}
 and $\hat{h}_{i}(x) = h(x)-\overline{h}_{\gamma_{i}}$. 
Suppose  $\gamma_{1},\ldots,\gamma_{m}$, and $\theta_{ij}$ for $i < j$ are chosen such that the following conditions are satisfied:
\begin{enumerate}
%\item   There exist class-K functions $\alpha_{1}^{i}$, $\alpha_{2}^{i}$: $i=1,\ldots,m$ such that 
%\begin{equation}
%\label{eq:FT-CBF1}
%\frac{1}{\alpha_{1}^{i}(\hat{h}_{i}(x))} \leq B_{i}(x) \leq \frac{1}{\alpha_{2}^{i}(\hat{h}_{i}(x))}.
%\end{equation}
%for all $x \in \mbox{int}(\mathcal{C})$
\item Define  $\Lambda_{i}(\hat{x}_{t,i}) = \frac{\partial h_{i}}{\partial x}(\hat{x}_{t,i})g(\hat{x}_{t,i})$. There exists $\delta > 0$ such that for any $X_{t}^{\prime} \subseteq X_{t}(\delta)$ satisfying $||\hat{x}_{t,i}-\hat{x}_{t,j}||_{2} \leq \theta_{ij}$ for all $i,j \in X_{t}^{\prime}$,  there exists $u$ such that
\begin{equation}
\label{eq:FT-CBF2}
\Lambda_{i}(\hat{x}_{t,i})u > 0
\end{equation}
for all $i \in X_{t}^{\prime}$.
\item For each $i$, when $r=r_{i}$, 
\begin{multline}
\label{eq:FT-CBF3}
Pr(||\hat{x}_{t,i}-\hat{x}_{t,i,j}||_{2} \leq \theta_{ij}/2 \ \forall j, ||\hat{x}_{t,i}-x_{t}||_{2} \leq \gamma_{i} \ \forall t)\\
 \geq 1-\epsilon.
\end{multline}
\end{enumerate}
Then $Pr(x_{t} \in \mathcal{C} \ \forall t) \geq 1-\epsilon$ for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$.
\end{theorem}



==> sections/Problem.tex <==
\section{Problem Formulation}\label{sec:formulation}
\subsection{System Model} We consider a nonlinear control system with state $x_{t} \in \mathbb{R}^{n}$ and input $u_{t} \in \mathbb{R}^{p}$ at time $t$. The state dynamics and the system output $y_{t} \in \mathbb{R}^{q}$ are described by the stochastic differential equations
% \begin{equation}
\begin{align}
    \label{eq:state-sde}
    dx_{t} &= (f(x_{t})+g(x_{t})u_{t}) \ dt + \sigma_{t} \ dW_{t}\\
    \label{eq:output-sde}
    dy_{t} &= (c x_{t} + a_{t}) \ dt + \nu_{t} \ dV_{t}
\end{align}
% \end{equation}
where $f: \mathbb{R}^{n} \rightarrow \mathbb{R}^{n}$ and $g: \mathbb{R}^{n} \rightarrow \mathbb{R}^{n \times p}$ are locally Lipschitz, $\sigma_{t} \in \mathbb{R}^{n \times n}$, $W_{t}$ is an $n$-dimensional Brownian motion, $c \in \mathbb{R}^{q \times n}$,  $\nu_{t} \in \mathbb{R}^{q \times q}$, and $V_{t}$ is a $q$-dimensional Brownian motion. A control policy $\mu$ is defined as a function $\mu:\{y_{t^{\prime}} : t^{\prime} \in [0,t)\}\rightarrow \mathbb{R}^p$, mapping from the sequence of outputs to an control input $u_t\in\mathbb{R}^p$ at each time $t$. The attack signal is denoted as $a_{t}$, which will be detailed in Section \ref{sec:threat}. 


% We denote the control policy as $\mu$ maps the sequence $\{y_{t^{\prime}} : t^{\prime} \in [0,t)\}$ to an input $u_{t}$ at each time $t$. 

The system is required to satisfy a safety constraint, which is specified as the positive invariance of a given safety region. 
\begin{definition}[Safety]
    \label{def:positive-invariance}
    A set $\mathcal{D} \subseteq \mathbb{R}^{n}$ is positive invariant under dynamics \eqref{eq:state-sde}, \eqref{eq:output-sde} and control policy $\mu$ if $x_0\in \mathcal{D}$ and $u_{t} = \mu(x_{t}) \ \forall t \geq 0$ imply that $x_t \in \mathcal{D}$ for all $t \geq 0$. 
    If $\mathcal{D}$ is positive invariant, then the system satisfies the safety constraint with respect to $\mathcal{D}$.
\end{definition}
We define the safety region as follows.  
%quote and describe
\begin{definition}[Safety Region]
The safety region of the system is a set $\mathcal{C} \subseteq \mathbb{R}^{n}$ defined by 
\begin{align}
    \label{eq:safe-region}
    \mathcal{C} = \{{x} : h({x}) \geq 0\}, \\ \mbox{int}(\mathcal{C}) = \{{x} : h({x}) > 0\}, \\ \partial \mathcal{C} = \{{x} : h({x}) = 0\}
\end{align}
where $h: \mathbb{R}^{n} \rightarrow \mathbb{R}$ is twice-differentiable on $\mathcal{C}$.
\end{definition}
We assume throughout the paper that $x_{0} \in \mbox{int}(\mathcal{C})$, i.e., the system is initially safe. 

\subsection{Threat Model} \label{sec:threat}
We consider the presence of an adversary, who can inject an arbitrary attack signal, denoted as $a_{t}\in \mathbb{R}^{q}$, to manipulate the system output at each time $t$. The adversary aims to bias the sensor measurements to drive the system towards unsafe region. The attack signal is constrained by $\mbox{supp}(a_{t}) \subseteq \mathcal{F}(r)$. Hence, if fault $r$ occurs, then the outputs of any of the sensors indexed in $\mathcal{F}(r_{i})$ can be arbitrarily modified by the fault. The sets $\mathcal{F}(r_{1}),\ldots,\mathcal{F}(r_{m})$ are known, but the value of $r$ is unknown. In other words, the set of possible faults is known, but the exact fault that has occurred is unknown to the controller. In the worst-case, one can enumerate all possible combinations of indices of sensors under attacks and formulate $\mathcal{F}(r)$. 

\subsection{Problem Formulation}
% Definition of CBF
% CBF -> NCBF (synthesis (AC semi-alg))
% Attack free CBF/NCBF -> Safety
% Adversarial case CBF/NCBF fails -> motivation and problem formulation
The Control Barrier Functions (CBFs) have been employed to ensure the safety of nonlinear systems, and are defined as follows. 
\begin{definition}
    \label{def: CBFs}
    A function $b$ is a control barrier function for \eqref{eq:state-sde} if there is a class-K function $\alpha$ such that, for all $x$ with $b(x) \geq 0$, there exists $u$ satisfying
    \begin{equation}
        \frac{\partial b}{\partial x} (f(x) + g(x) u) \geq -\alpha(b(x))
    \end{equation}
\end{definition}
The safety guarantee of CBFs can be found in \cite{ames2019control}. 
% CBF -> synth CBF (synthesis (AC semi-alg))
However, one may not always get a good CBF candidate since typically, CBFs are constructed using trial-and-error or domain knowledge. Polynomial CBFs are synthesized using Sum of Squares (SOS) \cite{clark2022semi,breeden2021high, dai2022convex, kang2023verification}. The CBFs parameterized by neural networks known as NCBFs are proposed in~\cite{dawson2022safe,dawson2023safe,liu2023safe}. 
% This challenging problem motivate recent researches to construct CBFs using techniques such as Sum-of-Squares (SOS) \cite{clark2022semi,breeden2021high, dai2022convex, kang2023verification}. 
% SOS ill posed sparsity. NCBF is better in 1,2,3... (More realistic/powerful tool NCBF)
% However, on one hand SOS programs are known with numerical issues such as sparsity and ill-conditioned \cite{kojima2005sparsity}. While this novel class of CBFs that are parametrized by neural networks (\emph{neural control barrier functions} or  NCBFs)~\cite{dawson2022safe,dawson2023safe,liu2023safe} is promising due to the universal representability \cite{hornik1989multilayer, csaji2001approximation} of neural networks. 
% CBF -> NCBF
We denote the NCBF with parameter $\theta$ as $b_{\theta}$. We define its corresponding region as $\mathcal{D}_{\theta} = \{x : b_{\theta}(x) \geq 0\}$. 
%We next provide definition of correctness and feasibility properties of a NCBF.
To guarantee the safety of system \eqref{eq:state-sde}, we require the NCBF $b_\theta$ to satisfy two properties. 
\begin{definition}[Correct NCBFs]
    \label{def:correctness}
    Given a safety region $\mathcal{C}$, the NCBF $b_{\theta}$ is correct if and only if $\mathcal{D}_{\theta}\subseteq \mathcal{C}$. 
\end{definition}
\begin{definition}[Feasible NCBFs]
    \label{def:feasibility}
    The NCBF $b_{\theta}$ is feasible if and only if $\forall x\in \partial\mathcal{D}$, $\exists u$ s.t. $\frac{\partial b}{\partial x} f(x) + g(x) u \geq 0$. 
\end{definition}
We say an NCBF is \emph{valid} if it is feasible and correct.

% Attack free CBF/NCBF -> Safety
% Adversarial case CBF/NCBF fails -> motivation and problem formulation
Upon now, we have introduced safety guarantee of NCBFs. However, robustness of NCBFs are less explored, especially, in adversarial environments. 
Sensor faults or attacks bias the state estimates of systems, lead to unwanted control input and eventually sabotage the safety guarantee of both CBFs and NCBFs. However, the NCBFs robust to sensor faults are not yet been explored. To mitigate the influence of sensor faults and attacks on systems utilizing NCBFs, we formally formulate the problem as follows.

We make the following assumption for the sensor fault scenario. 
\begin{assumption}
\label{assumption:sf}
The system \eqref{eq:state-sde}-\eqref{eq:output-sde} and the sensor fault patterns $\mathcal{F}(r_1),\ldots,\mathcal{F}(r_m)$ satisfy the conditions:
\begin{enumerate}
    \item The system is controllable. 
    \item For each $i,j \in \{1,\ldots,m\}$, the pair\\ $[\frac{\partial \overline{f}}{\partial x}(x,u), \overline{c}_{i,j}]$ is uniformly detectable.
\end{enumerate}
\end{assumption}
\begin{problem}
    Given a safety set $\mathcal{C}$ defined in \eqref{eq:safe-region} and a parameter $\epsilon \in (0,1)$, synthesize a correct and feasible NCBF $b_{\theta}(x)$ parameterized by $\theta$. Then construct a control policy to synthesize $u_{t}$ such that, for any fault $r \in \{r_{1},\ldots,r_{m}\}$, $Pr(x_{t} \in \mathcal{C} \ \forall t) \geq (1-\epsilon)$ when fault $r$ occurs. 
\end{problem}



==> sections/Related.tex <==
\section{Related Work}
% This challenging problem motivate recent researches to construct CBFs using techniques such as Sum-of-Squares (SOS) \cite{clark2022semi,breeden2021high, dai2022convex, kang2023verification}. However, numerical issues of SOS program such as sparsity and ill-conditioned problem are investigated in \cite{cotorruelo2021reference} \cite{kojima2005sparsity}.  

However, one may not always get a good CBF candidate since typically, CBFs are constructed using trial-and-error or domain knowledge. This challenging problem motivate recent researches to construct CBFs using techniques such as Sum-of-Squares (SOS) \cite{clark2022semi,breeden2021high, dai2022convex, kang2023verification}. 
% SOS ill posed sparsity. NCBF is better in 1,2,3... (More realistic/powerful tool NCBF)
However, on one hand SOS programs are known with numerical issues such as sparsity and ill-conditioned \cite{kojima2005sparsity}. While this novel class of CBFs that are parametrized by neural networks (\emph{neural control barrier functions} or  NCBFs)~\cite{dawson2022safe,dawson2023safe,liu2023safe} is promising due to the universal representability \cite{hornik1989multilayer, csaji2001approximation} of neural networks. 

==> sections/problem_v1.tex <==
\section{Preliminaries and Problem Formulation}\label{sec:formulation}
This section presents preliminary background on extended Kalman filters and stochastic CBFs.
We then describe the system and adversary models.
We finally state the problem studied in this paper.

\subsection{Preliminaries}

Consider a robotic system operated in benign environment as follows
\begin{align}
    \label{eq:state}
    dx_{t} &= (f(x_{t})+g(x_{t})u_{t}) \ dt + \sigma_{t} \ dW_{t}\\
    \label{eq:output}
    dy_{t} &= c x_{t}  \ dt + \nu_{t} \ dV_{t}
\end{align}
where $x_t\in\mathbb{R}^n$ is the system state, $y_t\in\mathbb{R}^q$ is the output, and $u_t\in\mathbb{R}^p$ is the control input at each time $t$. Functions $f: \mathbb{R}^{n} \rightarrow \mathbb{R}^{n}$ and $g: \mathbb{R}^{n} \rightarrow \mathbb{R}^{n \times p}$ are locally Lipschitz, $\sigma_{t} \in \mathbb{R}^{n \times n}$, $W_{t}$ is an $n$-dimensional Brownian motion. In addition, matrix $c \in \mathbb{R}^{q \times n}$,  $\nu_{t} \in \mathbb{R}^{q \times q}$, and $V_{t}$ is a $q$-dimensional Brownian motion.
The extended Kalman filter (EKF) for system \eqref{eq:state}-\eqref{eq:output} is then defined as 
\begin{equation}
    d\hat{x}_t = (f(\hat{x}_{t})+g(\hat{x}_{t})u_{t})\ dt + K_t(dy_{t} - c\hat{x}_t),
\end{equation}
where $K_t=P_tc^TR_t^{-1}$ is the Kalman gain, $R_t = \nu_t\nu_t^T$, and $\hat{x}_t$ is the state estimate. Positive definite matrix $P_t$ is the solution to 
\begin{equation*}
    \frac{dP}{dt} = A_tP_t+P_tA_t^T+Q_t-P_tc^TR_t^{-1}cP_t,
\end{equation*}
where $Q_t=\sigma_t\sigma_t^T$, $A_t=\frac{\partial \Bar{f}}{\partial x}(\hat{x}_t,u_t)$, and $\Bar{f}(x,u)=f(x)+g(x)u$.
We make the following assumption in this paper.

% \subsubsection{Extended Kalman Filter}
\begin{assumption}
\label{assumption:ekf}
The SDEs (\ref{eq:state})-(\ref{eq:output}) satisfy the conditions:
\begin{enumerate}
\item There exist constants $\beta_{1}$ and $\beta_{2}$ such that $\mathbf{E}(\sigma_{t}\sigma_{t}^{T}) \geq \beta_{1} I$ and $\mathbf{E}(\nu_{t}\nu_{t}^{T}) \geq \beta_{2} I$ for all $t$. 
\item The pair $[\frac{\partial \overline{f}}{\partial x}(x,u),c]$ is uniformly detectable.
% \item The system has $(p-1)$ redundancy, where $p>1$. 
\item Let $\phi$ be defined by $$\overline{f}(x,u)-\overline{f}(\hat{x},u) = \frac{\partial \overline{f}}{\partial x}(x - \hat{x}) + \phi(x,\hat{x},u).$$ Then there exist real numbers $k_{\phi}$ and $\epsilon_{\phi}$ such that $$||\phi(x,\hat{x},u)|| \leq k_{\phi}||x-\hat{x}||_{2}^{2}$$ for all $x$ and $\hat{x}$ satisfying $||x-\hat{x}||_{2} \leq \epsilon_{\phi}$. 
\end{enumerate}
\end{assumption} 
The accuracy of state estimate from EKF is given by the theorem below.
\begin{theorem}[\cite{reif2000stochastic}]
\label{theorem:EKF}
Suppose that the conditions of Assumption \ref{assumption:ekf} hold. Then there exists $\delta > 0$ such that $\sigma_{t}\sigma_{t}^{T} \leq \delta I$ and $\nu_{t}\nu_{t}^{T} \leq \delta I$. For any $0<\epsilon <1$, there exists $\gamma > 0$ such that $$Pr\left(\sup_{t \geq 0}{||x_{t}-\hat{x}_{t}||_{2} \leq \gamma}\right) \geq 1-\epsilon.$$ 
\end{theorem}
We finally introduce stochastic CBFs for the system (\ref{eq:state})--(\ref{eq:output}), along with its safety guarantee.
% \subsubsection{Stochastic CBFs}
\begin{theorem}[\cite{clark2020control}]
\label{theorem:SCBF}
    For the system (\ref{eq:state})-(\ref{eq:output}) with safety region defined by (\ref{eq:safe-region}), define
    $$\overline{b}^{\gamma} = \sup_{x,x^{0}}{\{b(\hat{x}) : ||x-x^{0}||_{2} \leq \gamma \text{ and } b(x^{0})=0\}}. $$
    Let $\hat{b}^\gamma(\hat{x}) := b(\hat{x})-\overline{b}^{\gamma}$ and $\hat{x}_{t}$ denote the EKF estimate of $x_{t}$.
    Suppose that there exists a constant $\delta > 0$ such that   
    whenever $\hat{b}(\hat{x}_{t}) < \delta$, $u_{t}$ is chosen to satisfy
    \begin{multline}
    \label{eq:SCBF-2}
    \frac{\partial b}{\partial x}(\hat{x}_{t})\overline{f}(\hat{x}_{t},u_{t}) - \gamma||\frac{\partial b}{\partial x}(\hat{x}_{t})K_{t}c||_{2} \\
    + \frac{1}{2}\mathbf{tr}\left(\nu_{t}^{T}K_{t}^{T}\frac{\partial^{2}b}{\partial x^{2}}(\hat{x}_{t})K_{t}\nu_{t}\right) \geq -\hat{b}^\gamma(\hat{x}_{t}).
    \end{multline}
    Then $Pr(x_{t} \in \mathcal{D} \ \forall t | \ ||x_{t}-\hat{x}_{t}||_{2} \leq \gamma \ \forall t) = 1$, where $\mathcal{D}=\{x\mid b(x)\geq 0\}$. 
\end{theorem}

% The proof of Theorem \ref{theorem:SCBF} is very similar to the proof of Theorem 7 from \cite{clark2021control} and is omitted due to space constraints.
The function $b$ satisfying inequality \eqref{eq:SCBF-2} is a \emph{stochastic control barrier function (SCBF)}.
SCBF specifies that as the state approaches the boundary, the control input is chosen such that the rate of increase of the barrier function decreases to zero. 
Hence Theorem \ref{theorem:SCBF} implies that if there exists an SCBF for a system, then the safety condition is satisfied with probability $(1-\epsilon)$ when an EKF is used as an estimator and the control input is chosen at each time $t$ to satisfy (\ref{eq:SCBF-2}).



\subsection{System Model} We consider a nonlinear stochastic robotic system with state $x_{t} \in \mathbb{R}^{n}$ and input $u_{t} \in \mathbb{R}^{p}$ at time $t$. The state dynamics and the system output $y_{t} \in \mathbb{R}^{q}$ are described by the stochastic differential equations
% \begin{equation}
\begin{align}
    \label{eq:state-sde}
    dx_{t} &= (f(x_{t})+g(x_{t})u_{t}) \ dt + \sigma_{t} \ dW_{t}\\
    \label{eq:output-sde}
    dy_{t} &= (c x_{t} + a_{t}) \ dt + \nu_{t} \ dV_{t}
\end{align}
% \end{equation}
A control policy $\mu:\{y_{t^{\prime}} : t^{\prime} \in [0,t)\}\rightarrow \mathbb{R}^p$ is a mapping from the sequence of outputs to a control input $u_t\in\mathbb{R}^p$ at each time $t$. The attack signal is denoted as $a_{t}$, which will be detailed in Section \ref{sec:threat}. 


% We denote the control policy as $\mu$ maps the sequence $\{y_{t^{\prime}} : t^{\prime} \in [0,t)\}$ to an input $u_{t}$ at each time $t$. 

The system is required to satisfy a safety constraint, which is specified as the positive invariance of a given safety region. 
\begin{definition}[Safety]
    \label{def:positive-invariance}
    A set $\mathcal{D} \subseteq \mathbb{R}^{n}$ is positive invariant under dynamics \eqref{eq:state-sde}, \eqref{eq:output-sde} and control policy $\mu$ if $x_0\in \mathcal{D}$ and $u_{t} = \mu(x_{t}) \ \forall t \geq 0$ imply that $x_t \in \mathcal{D}$ for all $t \geq 0$. 
    If $\mathcal{D}$ is positive invariant, then the system satisfies the safety constraint with respect to $\mathcal{D}$.
\end{definition}

We denote the safety region required by the safety constraint as
\begin{equation}\label{eq:safe-region}
    \mathcal{C}= \{{x} : h({x}) \geq 0\},
\end{equation} 
where $h: \mathbb{R}^{n} \rightarrow \mathbb{R}$ is twice-differentiable on $\mathcal{C}$.
We further let the interior and boundary of $\mathcal{C}$ be $\mbox{int}(\mathcal{C}) = \{{x} : h({x}) > 0\}$ and $\partial \mathcal{C} = \{{x} : h({x}) = 0\}$, respectively.
%quote and describe
% \begin{definition}[Safety Region]
% The safety region of the system is a set $\mathcal{C} \subseteq \mathbb{R}^{n}$ defined by 
% \begin{align}
%     \label{eq:safe-region}
%     \mathcal{C} = \{{x} : h({x}) \geq 0\}, \\ \mbox{int}(\mathcal{C}) = \{{x} : h({x}) > 0\}, \\ \partial \mathcal{C} = \{{x} : h({x}) = 0\}
% \end{align}
% where $h: \mathbb{R}^{n} \rightarrow \mathbb{R}$ is twice-differentiable on $\mathcal{C}$.
% \end{definition}
We assume that $x_{0} \in \mbox{int}(\mathcal{C})$, i.e., the system is initially safe. 
We further assume that Assumption \ref{assumption:ekf} holds for system \eqref{eq:state-sde}-\eqref{eq:output-sde}.

\subsection{Adversary Model} \label{sec:threat}
We consider the presence of an adversary, who can inject an arbitrary attack signal, denoted as $a_{t}\in \mathbb{R}^{q}$, to manipulate the system output at each time $t$. The adversary aims to bias the sensor measurements to drive the system towards unsafe region. The attack signal is constrained by $\mbox{supp}(a_{t}) \subseteq \mathcal{F}(r)$, where $r\in\{r_1,\ldots,r_m\}$ is the index of possible faults or attacks, $m$ is the total number of possible attack patterns, and $\mathcal{F}(r)\subseteq\{1,\ldots,q\}$ denotes the set of potentially compromised sensors under attack pattern $r$.
Hence, if fault $r$ occurs, then the outputs of any of the sensors indexed in $\mathcal{F}(r_{i})$ can be arbitrarily modified by the fault. The sets $\mathcal{F}(r_{1}),\ldots,\mathcal{F}(r_{m})$ are known, but the value of $r$ is unknown. In other words, the set of possible faults is known, but the exact fault that has occurred is unknown to the controller. In the worst-case, one can enumerate all possible combinations of indices of sensors under attacks and formulate $\mathcal{F}(r)$. 
In this paper, we make the following assumption on the adversary model. 
\begin{assumption}
\label{assumption:sf}
The system \eqref{eq:state-sde}-\eqref{eq:output-sde} and the sensor fault patterns $\mathcal{F}(r_1),\ldots,\mathcal{F}(r_m)$ satisfy the conditions: (i) The system is controllable, and (ii) For each $i,j \in \{1,\ldots,m\}$, the pair $[\frac{\partial \overline{f}}{\partial x}(x,u), \overline{c}_{i,j}]$ is uniformly detectable, where $\overline{c}_{i,j}$ is the corresponding matrix after removing sensors affected by $r_i$ and $r_j$ from matrix $c$.
\end{assumption}

\subsection{Problem Formulation}
% Definition of CBF
% CBF -> NCBF (synthesis (AC semi-alg))
% Attack free CBF/NCBF -> Safety
% Adversarial case CBF/NCBF fails -> motivation and problem formulation
% The Control Barrier Functions (CBFs) have been employed to ensure the safety of nonlinear systems, and are defined as follows. 
% \begin{definition}[\cite{clark2021verification}]
%     \label{def: CBFs}
%     A function $b$ is a control barrier function for \eqref{eq:state-sde} if there is a class-K function $\alpha$ such that, for all $x$ with $b(x) \geq 0$, there exists $u$ satisfying
%     \begin{equation*}
%         \frac{\partial b}{\partial x} (f(x) + g(x) u) \geq -\alpha(b(x)).
%     \end{equation*}
% \end{definition}
% The safety guarantee of CBFs can be found in \cite{ames2019control}. 
% % CBF -> synth CBF (synthesis (AC semi-alg))
% However, synthesizing CBFs is computationally expensive. When the system dynamics are polynomial, SOS-based approaches have been proposed to search for CBFs \cite{clark2022semi,breeden2021high, dai2022convex, kang2023verification}.
% To generalize the synthesis of CBFs to more complex systems, we focus on NCBFs in this paper. 

In this paper, we study the synthesis of fault tolerant stochastic neural control barrier functions (FT-SNCBF) for system \eqref{eq:state-sde}-\eqref{eq:output-sde} under sensor faults and attacks.
We further investigate how to synthesize control inputs with safety guarantees using the FT-SNCBFs.
We denote the FT-SNCBF with parameter $\theta$ as $b_{\theta}$. We define $\mathcal{D}_{\theta} = \{x : b_{\theta}(x) \geq 0\}$.
The problem studied in this paper is then stated as follows.
%We next provide definition of correctness and feasibility properties of a NCBF.
% To guarantee the safety of system \eqref{eq:state-sde}, we require the SNCBF $b_\theta$ to satisfy two properties. 
% \begin{definition}[Correct SNCBFs]
%     \label{def:correctness}
%     Given a safety region $\mathcal{C}$, the SNCBF $b_{\theta}$ is correct if and only if $\mathcal{D}_{\theta}\subseteq \mathcal{C}$. 
% \end{definition}
% \begin{definition}[Feasible SNCBFs]
%     \label{def:feasibility}
%     The SNCBF $b_{\theta}$ is feasible if and only if $\forall x\in \partial\mathcal{D}$, $\exists u$ s.t. $\frac{\partial b}{\partial x} f(x) + g(x) u \geq 0$. 
% \end{definition}
% We say an NCBF is \emph{valid} if it is feasible and correct.

\textbf{Problem Statement:} Given a safety set $\mathcal{C}$ defined in \eqref{eq:safe-region} and a parameter $\epsilon \in (0,1)$, synthesize an FT-SNCBF $b_{\theta}(x)$ parameterized by $\theta$, and then construct a control policy $\mu$ such that, for any fault pattern $r \in \{r_{1},\ldots,r_{m}\}$, $Pr(x_{t} \in \mathcal{C} \ \forall t) \geq (1-\epsilon)$ when fault $r$ occurs. 

% Attack free CBF/NCBF -> Safety
% Adversarial case CBF/NCBF fails -> motivation and problem formulation
% Upon now, we have introduced safety guarantee of NCBFs. However, robustness of NCBFs are less explored, especially, in adversarial environments. 
% Sensor faults or attacks bias the state estimates of systems, lead to unwanted control input and eventually sabotage the safety guarantee of both CBFs and NCBFs. However, the NCBFs robust to sensor faults are not yet been explored. To mitigate the influence of sensor faults and attacks on systems utilizing NCBFs, we formally formulate the problem as follows.


% \begin{problem}
%     Given a safety set $\mathcal{C}$ defined in \eqref{eq:safe-region} and a parameter $\epsilon \in (0,1)$, synthesize a correct and feasible NCBF $b_{\theta}(x)$ parameterized by $\theta$. Then construct a control policy to synthesize $u_{t}$ such that, for any fault $r \in \{r_{1},\ldots,r_{m}\}$, $Pr(x_{t} \in \mathcal{C} \ \forall t) \geq (1-\epsilon)$ when fault $r$ occurs. 
% \end{problem}


% \begin{definition}[SCBF]
% \label{Def:SCBF}
%     The function $h$ is a \emph{Stochastic Control Barrier Function (SCBF)} of the system, if for all $\hat{x}_t$ satisfying $h(\hat{x}_t)>0$ there exists $u_t$ s.t. $\forall z_t$ with $\|z_t\|\leq \gamma$ \eqref{eq:SCBF-2} is satisfied. 
% \end{definition}

